Laccolith: Hypervisor-Based Adversary Emulation with Anti-Detection

Advanced Persistent Threats (APTs) represent the most threatening form of attack nowadays since they can stay undetected for a long time. Adversary emulation is a proactive approach for preparing against these attacks. However, adversary emulation tools lack the anti-detection abilities of APTs. We introduce Laccolith, a hypervisor-based solution for adversary emulation with anti-detection to fill this gap. We also present an experimental study to compare Laccolith with MITRE CALDERA, a state-of-the-art solution for adversary emulation, against five popular anti-virus products. We found that CALDERA cannot evade detection, limiting the realism of emulated attacks, even when combined with a state-of-the-art anti-detection framework. Our experiments show that Laccolith can hide its activities from all the tested anti-virus products, thus making it suitable for realistic emulations.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tex/dynamic.tex <==
\section{Dynamic Description}
\label{sec:dynamic}
\vittorio{Sezione dinamica: dinamicizzare descrizione architetturale con i passi eseguiti da Marco (prima VMI, poi iniezione ecc), magari spezzandola in più parti in base ai vari passaggi. Info su Volatility, API kernel utilizzate. Cenni su framework attorno, shell di controllo ecc. Autonomous red teaming (sez. dopo implementazione) per spiegare flusso di lavoro}
\marco{Questa sezione continuerà a cambiare man mano che saranno sviluppate iterazioni su Laccolith, ad esempio di recente abbiamo implementato anche la REST API ed integrato MongoDB per la gestione delle connessioni. Quindi può essere utile, in generale, specificare a quale versione del progetto si fa riferimento; la lista delle releases si trova qui: https://github.com/Shotokhan/adversary-emulation/releases}

==> tex/old/abstract.tex <==
\begin{abstract}
Advanced Persistent Threats (APTs) represent the most threatening form of attack nowadays since they can stay undetected for a long time. Adversary emulation is a proactive approach for preparing against these attacks. However, adversary emulation tools lack the anti-detection abilities of APTs. 
We introduce Laccolith, a hypervisor-based solution for adversary emulation with anti-detection to fill this gap. We also present an experimental study to compare Laccolith with MITRE CALDERA, a state-of-the-art solution for adversary emulation, against five popular anti-virus products. We found that CALDERA cannot evade detection, limiting the realism of emulated attacks, even when combined with a state-of-the-art anti-detection framework. Our experiments show that Laccolith can hide its activities from all the tested anti-virus products, thus making it suitable for realistic emulations.
\end{abstract}

==> tex/old/acknowledgments.tex <==
\section*{Acknowledgments}
This work has been partially supported by the Italian Ministry of University and Research (MUR) under the programme ``PON Ricerca e Innovazione 2014-2020 – Dottorati innovativi con caratterizzazione industriale''.

==> tex/old/background.tex <==
\section{Background}
\label{sec:background}

\begin{comment}
%\vittorio{
%\begin{itemize}
%    \item Spostare info su MITRE ATT\&CK dall'introduzione al background
%    \item Spostare citazioni del background in related
%    \item Riportare info su Adversary Emulation dal background del paper ISSRE
%    \item Inserire figura che rappresenta uno degli APT (stile FIN6)
%\end{itemize}
%}

\vittorio{
\textbf{Contenuto:}
\begin{itemize}
    %\item \textbf{APT}: cos'è + descrizione esempio (con molte azioni) + spiegazione APT "di dominio" (e.g. finanziario ecc) tra cui scegliere quali simulare (specificando che ognuno si porta dietro le proprie tecniche di obfuscation)
    \item \textbf{MITRE ATT\&CK}: cos'è + come usarlo per modellare APT
    %\item \textbf{CTI?}
    \item \textbf{CALDERA}: cos'è e a cosa serve + architettura client/server + no anti-detection
    \item \textbf{Inceptor}: cos'è e a cosa serve
    \item \textbf{Post-exploitation}
\end{itemize}
}

%NIST defines advanced persistent threats (APT) as: ''\textit{an adversary with sophisticated levels of expertise and significant resources, allowing it through the use of multiple different attack vectors (e.g., cyber, physical, and deception), to generate opportunities to achieve its objectives which are typically to establish and extend its presence within the information technology infrastructure of organizations for purposes of continually exfiltrating information and/or to undermine or impede critical aspects of a mission, program, or organization, or place itself in a position to do so in the future; moreover, the advanced persistent threat pursues its objectives repeatedly over an extended period of time, adapting to a defender’s efforts to resist it, and with determination to maintain the level of interaction needed to execute its objectives}" \cite{NIST80039}. 



%Defending an infrastructure from an APT can be a really challenging task: securing the perimeter of the infrastructure itself may not be enough since, currently, there is no way to prevent the exploitation of every zero-day vulnerability or instantaneously patch software, nor to eliminate the intrinsic 'human vulnerability' that may result in passwords and sensitive data exposure \cite{MITREAnalytics}. APTs carry out targeted attacks with clear objectives and well-defined goals. Consequently, APTs are usually classified according to the domain they target, such as education, finance, government, and healthcare. Every \textit{domain-specific} APT has its own peculiarities, like the obfuscation techniques it uses to evade defense. 

%Due to the complexity of APT campaigns, it is necessary to adopt new strategies to minimize damage after they successfully penetrate the defense of a target infrastructure. In recent years, security strategies have begun to focus on \textbf{post-compromise adversary behavior}, to better understand, anticipate, and detect their actions. These strategies are based on an \textit{assume breach} paradigm, leveraging the information provided by open Cyber Threat Intelligence (CTI), i.e., information on the capabilities and intentions of attackers, and on the techniques adopted in their campaigns. \textbf{Adversary emulation} \cite{Applebaum2016IntelligentAR} is one of the most prominent among these approaches: it is based on the emulation attackers within an IT system for training and evaluation purposes.

\end{comment}

APTs are complex attack campaigns that eventually gain access to a target infrastructure due to inevitable weaknesses, such as the exploitation of an unknown (``zero-day'') software vulnerability, a known vulnerability in outdated software, or human mistakes that result in weak credentials, information disclosure, and execution of untrusted code \cite{MITREAnalytics}. Initial access represents just the preliminary part of the attack, followed by several other activities that depend on the objectives and skills of the attackers. 

In recent years, several models were introduced to describe the actions and behavior of attackers. 
ATT\&CK \cite{attack} is a security framework introduced by the MITRE Corporation and has rapidly become the \textit{de facto} standard in the security community. ATT\&CK provides a detailed classification of the adversaries' tactics, techniques, and procedures (TTPs), organized as a matrix, continuously updated by observing and analyzing threat intelligence sources \cite{strom2018mitre, zilberman2020sok}. \emph{Tactics} describe \textbf{why} an adversary performs an action, and \emph{techniques} describe \textbf{how} they do it. Techniques are described in the ATT\&CK model from both offensive and defensive points of view, so they are a useful reference and pivot between both disciplines. The descriptions also include references to known usage examples of the specific techniques and links to public threat reporting on adversary groups and their campaigns. Moreover, techniques can further specialize into sub-techniques, which usually provide more specific versions of an attacker's actions. Finally, \emph{procedures} represent the actual implementation of techniques for specific target systems.
At the time of writing, ATT\&CK encompasses 193 techniques and 401 sub-techniques. The richness of this framework makes it suitable for modeling APT campaigns. It is worth noting that a great number of combinations of TTPs is possible, making it relevant to focus on the TTPs of specific APTs of interest. Typically, APTs are classified according to the targeted domain, such as education, finance, government, and healthcare.

\begin{figure}[htbp]
\centering
\centerline{\includegraphics[width=\linewidth]{img/OilRig.png}}
\caption{OilRig Operational Steps. The \textcolor{red}{red dotted} arrows represent C2 communication, the black ones the operational steps.}
\label{fig:OilRig}
\end{figure}

As an example, we will refer to the OilRig APT \cite{oilrig}. OilRig is a cyber threat actor operating since 2014, interested in several domains, such as finance, government, energy, chemical, and telecommunications \cite{oilrigsummary}. It primarily leverages social engineering as an initial attack vector. The Center for Threat-Informed Defense (CTID) \cite{CTID} defined the model of its behavior and actions by collecting and analyzing threat and incident reports from several sources, such as Cyware \cite{Cyware}, Mandiant \cite{OilRigMandiant}, and Malwarebytes Labs \cite{Malwarebytes}. Figure \ref{fig:OilRig} shows OilRig's operational steps for \emph{exfiltrating data from a targeted server}. The first tactical goal is \emph{Initial Access}, to identify the target to exploit: OilRig achieves it using \emph{spearfishing attachment} (T1566\footnote{\textbf{Txxxx} indicates a technique from the MITRE ATT\&CK framework} \cite{T1566}) (step \circled{1} in Figure \ref{fig:OilRig}). Once the target opens the malicious attachment (T1204.002 \cite{T1204}), a backdoor is installed on the host machine (step \circled{2}). Then, it performs \emph{enumeration} (T1087 \cite{T1087}) (step \circled{3}), leading to the discovery that the user is a member of the administrator group on an Exchange Web Server (EWS). Using the aforementioned backdoor, OilRig \emph{obtains credentials} to EWS (T1003 \cite{T1003}) (step \circled{4}). Leveraging these credentials, the attackers connect to EWS and install a new backdoor (step \circled{5}) to perform further \emph{enumeration} (T1087 \cite{T1087}) (step \circled{6}): this leads to the discovery of an SQL server. Using the backdoor, OilRig \emph{dumps the credentials} (T1003 \cite{T1003}) (step \circled{7}) to access the SQL server. The next step is \emph{lateral movement} towards the server (step \circled{8}) by passing-the-hash (T1550.002 \cite{T1550}), where the attackers will copy the database backup files (step \circled{9}) and exfiltrate them to a controlled mailbox (T1048 \cite{T1048}) (step \circled{10}).

Once a model of an APT has been created using the ATT\&CK framework, it can be used for testing and assessing the security posture of a target infrastructure through adversary emulation. Several tools have been developed to facilitate and automate adversary emulation. They provide automated low-level procedures that implement the techniques described by the ATT\&CK framework. These procedures emulate the actions of actual adversaries in a typical attack scenario. In particular, we will refer to CALDERA \cite{Applebaum2016IntelligentAR, CALDERAGitHub}, an open-source adversary emulation tool developed by MITRE. CALDERA has gained popularity due to its feature-richness, maturity, and ease of setup and use \cite{zilberman2020sok}. In addition, it provides high coverage of TTPs of the MITRE ATT\&CK framework. In contrast, other adversary emulation tools consist of a small set of scripts (e.g., in Python and Powershell) that automate individual malicious actions (e.g., the Atomic Red Team), leaving human red teams to string these single actions into a complete APT campaign.

CALDERA is based on a client/server architecture, as shown in Figure \ref{fig:Adversary Emulation architecture}: the command-and-control (C2) server is responsible for administrating the operations, i.e., the simulations, planning the actions to execute, and making all the information available to the user. On the other hand, the clients are the agents installed on the target machines: the agent is responsible for the actual execution of the actions and for sending the results back to the C2 server. 
%However, CALDERA is not equipped with any anti-detection capability: this makes it not suitable for actual security assessment simulations since its activities are easily flagged by AVs/EDRs (red dotted arrow in Figure \ref{fig:Adversary Emulation architecture}). 

\begin{figure}[htbp]
\centering
\centerline{\includegraphics[width=\linewidth]{img/Adversary Emulation Architecture.png}}
\caption{Adversary emulation traditional architecture.}
\label{fig:Adversary Emulation architecture}
\end{figure}

Adversary emulation tools, such as CALDERA, do not provide anti-detection techniques but require the red teams to hide their traces using separate tools. A state-of-the-art toolkit for anti-detection is Inceptor \cite{Inceptor}. Inceptor is a well-known template-driven framework for AV evasion. A template is a generic, customizable loader with placeholders for evasion techniques and the actual payloads. There are many templates for three different types of payloads: .NET, PowerShell, and native code. Inceptor offers the possibility of chaining encoding techniques to evade static code analysis. It is also possible to plugin additional source code writing techniques to evade the Windows Antimalware Scanning Interface's (AMSI) dynamic analysis \cite{hendler2020amsi}. AMSI also analyses in-memory artifacts, for example, text areas the code is going to jump to. For this reason, Inceptor includes AMSI bypass techniques \cite{40}. 
In our experimental evaluation of the state-of-the-art on adversary emulation and anti-detection, we consider MITRE CALDERA in combination with Inceptor.

\begin{comment}

%In recent years, several tools have been developed to facilitate the adoption of adversary emulation and to automate most of the related activities. As mentioned in Section \ref{sec:introduction}, these tools' goal is to test and evaluate the security countermeasures of a target infrastructure. For this purpose, they provide sets of automated low-level procedures that implement the techniques described by MITRE in their ATT\&CK framework. These procedures aim to emulate the actions performed by actual adversaries in a typical attack scenario.

%Zilberman et al. \cite{Sok} analyze and classify several threat emulators. The authors define: a set of criteria and a methodology to evaluate the threat emulators; a taxonomy of the qualities of the threat emulators; and some guidelines for choosing the appropriate threat emulator, given the specific environment and the security assessment tasks. Among the criteria defined in this work are OS compatibility, changes needed in the security array, ATT\&CK TTPs coverage, procedures configuration, and required security expertise. 

%Examples of solutions are MITRE CALDERA \cite{Applebaum2016IntelligentAR}, Atomic Red Team \cite{AtomicRedTeam}, Infection Monkey \cite{InfectionMonkey}, and Red Team Automation \cite{RedTeamAutomation}. All of these solutions were ranked as the leading among those analyzed by Zilberman et al. \cite{Sok}. With respect to overall criteria, CALDERA can be defined as the most prominent and detailed. It has gained high popularity due to its ease of setup and use. In addition, it is characterized by a high level of detail, in terms of coverage of ATT\&CK TTPs. 

%\subsection{System/attacker model}
%\vittorio{Spiegare cosa può/non può fare l'attacker che vogliamo emulare}


The planning and execution of adversary emulation exercises are expensive activities, in terms of skills and man-hours to invest. They include teaming as well as other activities: scenario definition, monitoring, and results evaluation.
Adversary emulation is composed of a set of activities that can be split into two macro-phases: \textit{Attack modeling} and \textit{Attack emulation}.

\vspace{3pt}
\noindent
\textbf{Attack modeling}. This phase concerns Cyber Threat Intelligence and it gathers information on the threats and attacks to emulate. A significant effort is required to gather these documents, because of their heterogeneous nature and sources. It is then necessary to analyze and systematize this data, to map an attack onto a set of operational steps, to define an execution flow for the emulation exercise. 
To this goal, many cybersecurity frameworks provide taxonomies of attack tactics, techniques, and procedures (TTPs), with MITRE ATT\&CK \cite{attack} rapidly becoming the \textit{de facto} standard in the cybersecurity landscape. 
All the activities required by this phase are currently performed by human operators, hence the need for highly specialized personnel.

\vspace{3pt}
\noindent
\textbf{Attack emulation}. The second macro-phase of adversary emulation is the operational execution of the attack, leveraging the information provided by the previous phase. The attack techniques must be associated with implementation, provided by specific threat emulator tools.
Among these emulators, MITRE CALDERA \cite{Applebaum2016IntelligentAR, CALDERAGitHub} is the most prominent one, as it is designed for orchestrating complex attacks that consist of multiple techniques. 

A threat emulator needs to be configured before running a simulation: we will refer to CALDERA to describe the necessary steps. First of all, it is necessary to set up the Command and Control server, which will coordinate the simulations. The next step is to deploy the remote agent on the target machine: an agent is a software program that connects to the C2 server via a predefined contact method \cite{CALDERAdocs}. The C2 server will be responsible for sending the instructions to the agents. Once the agent has been deployed, it is possible to choose the \textit{adversary profile} for the simulation. A profile is a group of abilities that includes the attack techniques typically used by a specific attacker \cite{CALDERAdocs}.

In the case of FIN6, a new adversary profile for CALDERA needs to be configured, by combining multiple techniques from CALDERA into an orchestrated attack. Therefore, the emulation of an attack relies on accurate planning of adversarial activities, which is currently performed by human operators. To overcome this issue, it is helpful to automate the analysis of CTI, by extracting adversary techniques and mapping them to a standard taxonomy (e.g., MITRE ATT\&CK) to feed the emulation tool.
\end{comment}

==> tex/old/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we presented Laccolith, a hypervisor-based solution for adversary emulation equipped with anti-detection capabilities. Laccolith introduces a new approach to inject an agent into the target machine based on virtualization, an enabling technology for cybersecurity assessment and training infrastructures.
In addition, we performed an experimental analysis to compare Laccolith with MITRE CALDERA, a state-of-the-art solution for adversary emulation. Our analysis showed that CALDERA cannot evade detection by AV/EDR solutions, limiting its adoption for security assessment and training purposes. We also integrated CALDERA with anti-detection solutions, namely Inceptor, to find out that this combination was still unable to evade defense mechanisms. Instead, Laccolith evaded all the AVs for both the injection and emulation phases with high reliability, making it suitable for usage in actual emulation scenarios.

==> tex/old/dynamic.tex <==
\section{Dynamic Description}
\label{sec:dynamic}
\vittorio{Sezione dinamica: dinamicizzare descrizione architetturale con i passi eseguiti da Marco (prima VMI, poi iniezione ecc), magari spezzandola in più parti in base ai vari passaggi. Info su Volatility, API kernel utilizzate. Cenni su framework attorno, shell di controllo ecc. Autonomous red teaming (sez. dopo implementazione) per spiegare flusso di lavoro}
\marco{Questa sezione continuerà a cambiare man mano che saranno sviluppate iterazioni su Laccolith, ad esempio di recente abbiamo implementato anche la REST API ed integrato MongoDB per la gestione delle connessioni. Quindi può essere utile, in generale, specificare a quale versione del progetto si fa riferimento; la lista delle releases si trova qui: https://github.com/Shotokhan/adversary-emulation/releases}

==> tex/old/experiment.tex <==
\section{Experimental Analysis}
\label{sec:experiment}
%In this section, we present an experimental analysis on:
%\begin{itemize}
%    \item \textit{Detectability evaluation of popular adversary emulation tools}: we studied the detectability of MITRE CALDERA as standalone and then in combination with Inceptor, introduced in Section \ref{sec:background};
%    \item \textit{Detectability evaluation of Laccolith}: we repeated the detectability analysis with Laccolith to compare it with CALDERA;
%    \item \textit{Reliability of the injection method}: w.
%\end{itemize}
We compare Laccolith with MITRE CALDERA since it is a state-of-the-art solution for adversary emulation. Compared to other adversary emulation tools, CALDERA provides greater coverage of APT tactics and techniques, a complete client-server architecture, and the ability to orchestrate complex APT campaigns (see also  Section~\ref{sec:related} for a detailed comparison). We evaluate adversary emulation concerning its \textit{detectability}.

To evaluate detectability, we test the adversary emulation tools against a set of AV solutions, described in Section~\ref{sec:Experimental Setup}. 
As a metric to measure detectability, we consider the \textbf{adversary profile execution progress}. An adversary profile is a sequence of atomic steps which represent malicious activities. The metric represents the progress of the execution of an adversary profile in terms of atomic steps successfully executed until the AV raises an alarm. The \textit{successful execution} of an atomic step means that the agent (from either CALDERA or Laccolith) can execute the action without being detected by the AV. The steps that compose an adversary profile are called \textit{abilities} for CALDERA and \textit{actions} for Laccolith.
This metric is expressed as a fraction:
\begin{displaymath}
%\centering
    \textrm{Adversary Profile Execution Progress \hspace{3pt}} = \textrm{\hspace{5pt}} \frac{N_{EA}}{N_{PA}} 
\end{displaymath}
$N_{EA}$ is the number of executed actions of an adversary profile, while $N_{PA}$ is the total number of its actions. For example, suppose a profile has 10 actions, and the AV detects the execution of its eighth action. In that case, the adversary profile execution progress will be $7/10$ since the profile managed to execute 7 actions out of 10.

To gain additional insights into the detectability, we also analyze the initial loading of the emulation agent in the victim machine. Since AV products perform rigorous checks before an executable launches, the emulation agent also needs to evade these checks. For this purpose, we introduce an additional metric, the \textbf{injection success}. This metric represents the probability of successfully injecting the agent into the victim without triggering detection. 
The metric is defined as a fraction:
\begin{displaymath}
    \textrm{Injection Success \hspace{3pt}} = \textrm{\hspace{5pt}} \frac{N_{SI}}{N_{I}} 
\end{displaymath}
where $N_{SI}$ is the number of successful injections attempts and $N_{I}$ is the total number of attempts.

%We introduce this new metric since the injection phase is a critical phase of adversary emulation: analyzing this phase is helpful to get insight into the effectiveness of the proposed approach in emulating the behavior of APTs.



\subsection{Experimental Setup}
\label{sec:Experimental Setup}

We used the following configuration for the experimental analysis, shown in Figure~\ref{fig:Setup}:
\begin{itemize}
    \item Victim Windows 10 VM (VM1): the target of the adversary emulation;
    \item Additional Windows 10 VM (VM2): it is a machine necessary to perform some malicious actions, e.g., network shares enumeration performed by the \textit{Shares Hunter} profile, as shown in Table \ref{tab:Laccolith profiles}.
\end{itemize}

Both VMs are equipped with 4 CPU cores and 2 GB RAM and run Microsoft Windows 10. Before our experiments, we tested the portability of Laccolith across different versions of the guest OS. We deployed Laccolith on seven Windows 10 versions, which span over three years, with significant changes across the versions \cite{26}. 
Laccolith leverages Volatility to apply the injection method in a portable way. Indeed, Laccolith could correctly inject the emulation agent in all the tested versions of Windows without the need for special customizations. In our experiments, we focus on Microsoft Windows 10 build 19044.
%\vittorio{Descrivere quante version di Windows abbiamo testato e quanto tempo spaziano queste versioni}

%\textcolor{red}{Puoi indicare "Linux host with KVM/QEMU hypervisor"}
%19041.1415 (14/12/21), 19044.1706(10/05/22), 19044.1889 (09/08/22), 19044.2006 (13/09/22), 19044.2130 (11/10/22), 19044.2364 (13/12/22), 19044.2486 (10/01/23)
%\textcolor{red}{puoi aggiungere qualche info sul ruolo di queste tre macchine? Victim è il target della iniezione, VM2 è coinvolta in alcune malicious activities (qualche esempio..), gateway ti serve per coordinare? Cerca di arrangiare gli elementi della figura per ridurre lo spazio bianco. Fornisci qualche informazione sulla dotazione hardware e sulle versioni del software.}


%\textcolor{red}{Riguardo la versione di Windows OS: dire che abbiamo estensivamente testato Laccolith su varie versioni di Windows, sfruttando il supporto fornito da Volatility per ottenere la portabilità, e che il tool è stato in grado di eseguire correttamente in tutti i casi. Possiamo specificare la build di Windows su cui abbiamo fatto gli esperimenti.}

\begin{figure}[!htbp]
\centering
\centerline{\includegraphics[width=1\columnwidth]{img/Experimental Setup.png}}
\caption{Experimental setup.}
\label{fig:Setup}
\end{figure}

We selected five popular AV products for our detectability analysis: Windows Defender, Avast, AVG, Kaspersky, and Avira. These products qualify as modern EDR solutions and cover state-of-the-art detection techniques \cite{botacin2022antiviruses}. For instance, they monitor system calls using user-space and kernel-space hooks; they use both signature-based and real-time behavioral detection; and they implement self- and system-protection techniques. An example of such protections is preventing filesystem access to specific directories, such as the main system directories and the AV directory itself. %\textcolor{red}{hai qualche esempio di protection technique?}

%\textcolor{red}{Chiarire che AV scelti sono prodotti sofisticati e che usiamo AV come terminologia "estesa"}

\subsection{Detectability evaluation of MITRE CALDERA}
To study the detectability of CALDERA, we selected its twelve default adversary profiles. These profiles can be classified into two categories: \textit{reconnaissance \& information gathering} and \textit{advanced}. The first category encompasses the first eight profiles listed below, which perform basic operations: user identification, process enumeration, anti-virus discovery, screenshot capture, and file search. The advanced profiles perform more invasive actions, like process injection, lateral movement, and malicious payload execution. As a consequence, their activities will be noisy and more likely to be flagged by the anti-viruses. We report a short description for each profile:
\begin{itemize}
    \item \textit{Discovery}: collects detailed information from a host, such as local users, user processes, admin shares, and anti-virus programs;
    \item \textit{Hunter}: performs Discovery operations, then tries to exfiltrate files from the working directory;
    \item \textit{Check}: collects information about the configuration of the host (e.g., installation of common software packages, such as Chrome, Go, and Python), and the configuration of its network interfaces;
    \item \textit{Collection}: collects personal information from the host, such as company emails, IP addresses, and personal files;
    \item \textit{Enumerator}: enumerates the presence of different types of processes on the host, such as WMIC, PowerShell, and SysInternals utilities;
    \item \textit{Nosy Neighbor}: finds the preferred Wi-Fi networks, and tries to disrupt the Wi-Fi connection;
    \item \textit{Signed Binary Proxy Execution}: executes malicious code through signed and trusted binaries;
    \item \textit{Super Spy}: monitors the active user by capturing screenshots, copying data from the clipboard, and scanning preferred Wi-Fi networks;
    \item \textit{Undercover}: swaps the built-in PowerShell with PowerShell Core to stop PowerShell processes;
    \item \textit{Stowaway}: injects Sandcat (the default emulation agent in CALDERA) into another process;
    \item \textit{Worm}: runs PowerKatz to steal user credentials, then moves laterally in multiple ways;
    \item \textit{You Shall (Not) Bypass}: bypasses User Account Control (UAC).
\end{itemize}

%\vittorio{Noi dobbiamo avere/abbiamo due categories di profiles, spiegare prima le categorie e poi introdurre i profili che vengono analizzati}
In addition to these profiles, we implemented a custom \textit{Ransomware} profile for completeness. This profile was developed from scratch, similar to the implementation of the predefined profiles. It encompasses the following abilities:
\begin{itemize}
    \item Find files;
    \item Stage sensitive files;
    \item Compress the staged directory;
    \item Exfiltrate the staged directory;
    \item Encrypt sensitive files (e.g., \textit{docx} and \textit{pdf} files).
\end{itemize}

%\textcolor{red}{qualche esempio di sensitive file? docx?}
The first four abilities re-use the ones of the predefined profiles to find the target files. The last ability has been implemented with a PowerShell script \cite{56} to encrypt the sensitive files, by silently skipping the files if it does not have permission to rewrite them. Using a PowerShell script with standard APIs for encryption makes the process more similar to ``legitimate'' programs (as in fileless malware), similar to other profiles in CALDERA. In this way, the Ransomware profile should be as detectable as the other reconnaissance \& information gathering adversary profiles.
%This also weakens the encryption process, since PowerShell may log commands, thus leaking helpful information to recover the files.

%\marco{Notare che per il profilo ransomware su caldera è stata fatta un'analisi carta e penna, infatti c'è scritto "is expected", quindi quel 5/5 nella tabella si potrebbe contrassegnare con un asterisco. \textbf{L'analisi è stata eseguita studiando la sequenza di comandi e verificando se fossero stati rilevati nelle campagne precedenti}}

\begin{table}[!ht]
\centering
\caption{Adversary Profile Execution Progress for MITRE CALDERA. \textcolor{red}{\textbf{Bold}} values represent incomplete progress.}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{Profile} & \textbf{Windows Defender} & \textbf{Avast} & \textbf{AVG} & \textbf{Kaspersky} & \textbf{Avira}\\
\hline
Discovery & \DrawPercentageBar{1} \hspace{7pt} 9/9 & \DrawPercentageBar{1} \hspace{7pt} 9/9 & \DrawPercentageBar{1} \hspace{7pt} 9/9 & \DrawPercentageBar{1} \hspace{7pt} 9/9 & \DrawPercentageBar{1} \hspace{7pt} 9/9 \\
\hline
Hunter & \DrawPercentageBar{1} 14/14 & \DrawPercentageBar{1} 14/14 & \DrawPercentageBar{1} 14/14 & \DrawPercentageBar{1} 14/14 & \DrawPercentageBar{1} 14/14 \\
\hline
Check & \DrawPercentageBar{1} \hspace{7pt} 6/6 & \DrawPercentageBar{1} \hspace{7pt} 6/6 & \DrawPercentageBar{1} \hspace{7pt} 6/6 & \DrawPercentageBar{1} \hspace{7pt} 6/6 & \DrawPercentageBar{1} \hspace{7pt} 6/6 \\
\hline
Collection & \DrawPercentageBar{1} \hspace{7pt} 2/2 & \DrawPercentageBar{1} \hspace{7pt} 2/2 & \DrawPercentageBar{1} \hspace{7pt} 2/2 & \DrawPercentageBar{1} \hspace{7pt} 2/2 & \DrawPercentageBar{1} \hspace{7pt} 2/2 \\
\hline
Enumerator & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 \\
\hline
Nosy Neighbor & \DrawPercentageBar{1} \hspace{7pt} 7/7 & \DrawPercentageBar{1} \hspace{7pt} 7/7 & \DrawPercentageBar{1} \hspace{7pt} 7/7 & \DrawPercentageBar{1} \hspace{7pt} 7/7 & \DrawPercentageBar{1} \hspace{7pt} 7/7 \\
\hline
Signed Binary Proxy Execution & \DrawPercentageBar{1} \hspace{7pt} 3/3 & \DrawPercentageBar{1} \hspace{7pt} 3/3 & \DrawPercentageBar{1} \hspace{7pt} 3/3 & \DrawPercentageBar{1} \hspace{7pt} 3/3 & \DrawPercentageBar{1} \hspace{7pt} 3/3 \\
\hline
Super Spy & \DrawPercentageBar{1} 11/11 & \DrawPercentageBar{1} 11/11 & \DrawPercentageBar{1} 11/11 & \DrawPercentageBar{1} 11/11 & \DrawPercentageBar{1} 11/11 \\
\hline
Undercover & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{1} \hspace{7pt} 2/2 \\
\hline
Stowaway & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{1/2}} & \DrawPercentageBar{1} \hspace{7pt} 2/2 \\
\hline
Worm & \DrawPercentageBar{0.1111} \hspace{10pt} \textcolor{red}{\textbf{1/9}} & \DrawPercentageBar{0.1111} \hspace{10pt} \textcolor{red}{\textbf{1/9}} & \DrawPercentageBar{0.1111} \hspace{10pt} \textcolor{red}{\textbf{1/9}} & \DrawPercentageBar{0.1111} \hspace{10pt} \textcolor{red}{\textbf{1/9}} & \DrawPercentageBar{1} \hspace{7pt} 9/9 \\
\hline
You Shall (Not) Bypass & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{2/4}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{2/4}} & \DrawPercentageBar{0.5} \hspace{10pt} \textcolor{red}{\textbf{2/4}} & \DrawPercentageBar{0.25} \hspace{10pt} \textcolor{red}{\textbf{1/4}} & \DrawPercentageBar{0.25} \hspace{10pt} \textcolor{red}{\textbf{1/4}} \\
\hline
Ransomware & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 & \DrawPercentageBar{1} \hspace{7pt} 5/5 \\
\hline
\end{tabular}%
}
\label{tab:CALDERA profile progress}
\end{center}
\end{table}

%\textcolor{red}{aggiungiamo qui una frase, per dire che il solo caricamento di CALDERA viene già rilevato dagli anti-virus, e che abbiamo fatto ulteriori analisi assumendo che CALDERA sia stato già caricato.}
Table \ref{tab:CALDERA profile progress} shows the execution progress for each adversary profile of MITRE CALDERA against the five anti-viruses. 
It is possible to notice that the reconnaissance \& information gathering profiles execute without being detected since they do not perform harmful actions. For the advanced profiles, the results of the experiments are quite different. During the execution, all the anti-viruses, except for Avira, flagged the activities of the profiles as suspicious. Moreover, the detected abilities are always the first ones in the atomic order: once an ability has been detected, it is not possible to complete the operation, since the prerequisites for the following ones will not be satisfied. As a consequence, the last abilities of the advanced profiles could not be executed. For instance, the Stowaway profile uses two abilities: since the execution of the first one is stopped by the anti-virus, the second one cannot be tested. Therefore, this profile scored $1/2$ in terms of detectability. We reported the detected abilities for each profile in Table \ref{tab:Detected abilities}. 
This experimental analysis shows that the emulation agent of MITRE CALDERA can stealthily execute most Discovery, Collection, and Exfiltration techniques, but is easily blocked when it tries to perform more intrusive actions, such as Credential Access and Privilege Escalation.

\begin{table*}[ht]
\caption{Abilities of MITRE CALDERA detected by AV products.}
\begin{center}
\begin{tabular}{ccccccc}
\hline
\textbf{Profile} & \textbf{Ability} & \textbf{Windows Defender} & \textbf{Avast} & \textbf{AVG} & \textbf{Kaspersky} & \textbf{Avira}\\
\hline
Undercover & Install PowerShell Core 6 & \ding{51} & \ding{51} & \ding{51} & \ding{51} &\\
\hline
Stowaway & Inject Sandcat into Process & \ding{51} & \ding{51} & \ding{51} & \ding{51} &\\
\hline
Worm & Run PowerKatz & \ding{51} & \ding{51} & \ding{51} & \ding{51} &\\
\hline
You Shall (Not) Bypass & Wow64log DLL Hijack & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51}\\
\hline
You Shall (Not) Bypass & Bypass UAC Medium & \ding{51} & \ding{51} & \ding{51} & &\\
\hline
\end{tabular}
\label{tab:Detected abilities}
\end{center}
\end{table*}

It is worth noting that the AVs always detect the injection of CALDERA's agent. After performing 20 repetitions of the injection, we conclude that the injection success of CALDERA is $0/20$ against each AV. Consequently, the results in Table \ref{tab:CALDERA profile progress} only refer to the execution of the adversary profiles, assuming that the agent has already been loaded on the target machine.

\subsubsection{Integrating CALDERA with anti-detection}

To overcome the limitations of MITRE CALDERA in terms of anti-detection, we combined it with Inceptor \cite{Inceptor}, a state-of-the-art evasion framework introduced in Section~\ref{sec:background}. 
In this experimental analysis, we focus on Windows Defender, and on the injection stage of the emulation agent of CALDERA (i.e., the initial installation of the agent). We enhance the agent with multiple anti-detection techniques from Inceptor. 

The injection needs to bypass three layers of detection: User Account Control (UAC), signature-based static analysis, and dynamic sandbox analysis. UAC is a protection that involves user interaction, by displaying a message through a GUI frontend (Microsoft SmartScreen \cite{SmartScreen}). Sandbox analysis is a technique used by anti-virus software to analyze potentially malicious files and programs, by running them in a safe and isolated environment. It is particularly useful for detecting new and unknown malware, which can often evade static signature-based detection. In Microsoft Windows, \textit{Windows Defender Application Guard} \cite{ApplicationGuard} is responsible for performing the sandbox analysis, using a virtual container with a specialized version of the Windows OS.

We used the following combination of anti-detection techniques to make the injection stealthier: a native binary template, an encoding chain composed of \textit{Shikata-Ga-Nai} \cite{Shikata}, a popular polymorphic binary encoder \cite{ShikataMandiant}, XOR encoding, 120 seconds of execution delay, and an unhooking technique for EDR bypass. Moreover, we signed the resulting binary with a Microsoft signature using CarbonCopy \cite{41}.

We experimentally evaluate the injection of the CALDERA agent with anti-detection by performing 20 repetitions. The injection is unable to evade UAC. This would require the exploitation of known vulnerabilities in Microsoft Windows (\emph{UAC bypass}), which are regularly fixed by updates of the OS. Therefore, Inceptor is unable to provide a reliable solution to escape UAC, and we manually allow the execution of the CALDERA agent through the UAC. 
Even neglecting the problem with UAC, the agent was successfully injected approximately 5 times out of 20, thus with an injection success equal to $5/20$ and 25\% probability. %\textcolor{red}{Inserire esplicitamente che Injection Success è pari a 5/20 con conseguente probabilità} 
The encoding chain allows the binary to bypass static analysis since it does not match any known signature. The execution delay and unhooking technique heuristically help to elude the dynamic sandbox analysis: the delay is helpful to make the behavior seem benign while unhooking prevents EDRs from inspecting function calls.
The binary signature helped to evade the dynamic analysis: when the binary has a valid signature, Windows Defender performs less detailed dynamic checks. However, since the binary needs to decode itself from the encryption chain at some point, it is still challenging to bypass the sandbox analysis, making the injection detectable. 
The need for additional UAC bypass techniques further complicates the process of making CALDERA stealthier.


\begin{comment}
\textcolor{red}{Since all combinations except one were blocked either with static or dynamic analysis, we decided to report only the 'almost successful' combination.
This combination used: a native binary template, an encoding chain composed of Shikata-Ga-Nai \cite{Shikata} and XOR encoding, 120 seconds of execution delay, and an unhooking technique for EDR bypass. Moreover, the resulting binary was signed by Microsoft using CarbonCopy \cite{41}.
Our experimentation shows that binary templates perform better, the encoding chain is useful to bypass static analysis, whereas the execution delay and unhooking technique heuristically help to bypass the dynamic analysis. The crucial addition was the binary signature: if the binary has a valid signature, the dynamic analysis performed is less detailed.
With this combination, the agent was successfully injected approximately 1 time out of 4, with a 25\% probability (with some margin of error). Even though we did not perform a complete empirical study, we can state that the injection is only 'almost successful' because, even when not detected by Windows Defender, it still needs to bypass the UAC (Microsoft SmartScreen). 
Indeed, the binary is executed only after UAC approval, and even after that it still has an approximate probability of being executed as low as 25\%. The UAC approval mitigates the severity of this injection technique because it either requires user interaction or previous access that implemented UAC bypass and execution techniques.
To make things more clear: when the executable starts, the user sees Microsoft’s SmartScreen, which is the front-end to the UAC; if UAC approval is manually given, then the next ring in the necklace is Microsoft Defender, which performs an initial static analysis to check if the executable matches a known signature, then it performs dynamic analysis in a sandbox. This dynamic analysis is almost always successful in detecting the malicious code because it performs the signature match after decoding the packed malicious executable. Some helpful techniques against the dynamic analysis are the unhook technique to prevent EDRs from 'sniffing' on function calls, execution delay of the malicious part to make the behavior look good (before the decoding), and a valid signature for the executable, which reduces the overall amount of dynamic analysis performed. Therefore, after UAC approval/bypass, the behavior is still not deterministic: only approximately 25\% times the executable manages to bypass all controls performed by Microsoft Defender.}
\end{comment}

%\textbf{Servirebbe una soluzione aggiuntiva oltre ad Inceptor per UAC bypass, in quanto Inceptor si occupa solo di AV/EDR evasion. 1/4 è a valle di tutta la pipeline statica -> UAC -> dinamica}

\subsection{Detectability evaluation of Laccolith}
%\marco{Qui sono descritti a parole 3 profili, anche se poi nelle tabelle ne abbiamo aggiunto un quarto, "Shares Hunter" (che ha similitudine con il profilo "Worm" di Caldera); inoltre, nella tabella che descrive i profili, shares hunter ha 4 actions, mentre nell'esperimento ne ha 7. Questo si giustifica mediante il fatto che per tale profilo non si fa un planning a priori, ma c'è una parte di dynamic planning in cui le azioni successive dipendono dagli outcome delle azioni precedenti (come descritto nell'introduzione del paper). Quindi bisogna descrivere la configurazione specifica in cui abbiamo testato tale adversary profile, ovvero: una rete con (1) la VM target win10 (vm1), (2) il gateway (G), (3) un'altra VM win10 (vm2) con cui la vm1 ha interagito di recente (e quindi la vm1 ha l'indirizzo IP di vm2 nella ARP cache, oltre ovviamente a quello di G). Sia la vm1 sia la vm2 hanno il servizio di sharing con netbios attivo.}

Our previous analysis showed that traditional adversary emulation is cumbersome and unable to perform intrusive actions without being detected. We here present an experimental analysis of detectability for Laccolith. For this analysis, we implemented four adversary profiles with Laccolith: \textit{Thief}, \textit{Op-2}, \textit{Ransomware}, and \textit{Shares Hunter}, as described in Table \ref{tab:Laccolith profiles}. Since we had to develop adversary profiles from scratch for Laccolith, we did not aim for a verbatim reimplementation of the adversary profiles of CALDERA. Instead, the adversary profiles in Laccolith match the CALDERA profiles in terms of high-level strategy of the attackers. Moreover, we relate the adversary profiles for Laccolith with real-world APTs (threat-informed adversary emulation). The new profiles in Laccolith cover all the tactics covered by CALDERA profiles, except Privilege Escalation (covered by the \textit{You Shall (Not) Bypass} profile) since Laccolith already has high privilege. The Ransomware profile also covers the Impact tactic, which is not covered by the default profiles of CALDERA. We introduced this profile to show the ability of Laccolith to support complex operations and cover a relevant cybersecurity threat.

\begin{table*}[ht]
\centering
\caption{Adversary profiles in Laccolith.}
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{Profile} & \textbf{Description} & \textbf{Tactics} & \textbf{Commands} & \textbf{High-level actions} & \textbf{Referenced APTs}\\
\hline
& Exfiltrate files & Discovery, & Directory listing (to find & (1) Find local users, & APT1,\\
Thief & from local & Collection, & local users and to list & (2) List user desktop, & OilRig,\\
& user desktop & Exfiltration & desktop files), Read file & (3) Exfiltrate a list of staged files & APT3\\
\hline
& Upload a Powershell script & & & (1) Write file on &\\
& in a system folder & & Write file, & remote file system, &\\
& and install a scheduled & Persistence, & Write to registry, & (2) Install a scheduled & Remsec\\
Op-2 & task that executes that & Credential & Version, & task on the remote & (Strider),\\
& script at boot, get & access & Dump process & Windows target, & Ke3chang\\
& system version and & & memory & (3) Get system version, &\\
& dump LSASS memory & & & (4) Dump lsass credentials &\\
\hline
& & &  & (1) Find local users, &\\
& Discover and exfiltrate & Discovery, & Directory listing, & (2) Find sensitive files, & APT3,\\
Ransomware & sensitive files, encrypt & Collection, & Read file, & (3) Exfiltrate a list of staged & Bad Rabbit\\
& them and leave & Exfiltration, & Write file & files and encrypt them, & (multiple APTs)\\
& a message & Impact & & (4) Encrypt remote files, &\\
& & & & (5) Write ransom message &\\
\hline
& Read ARP cache to find & & & (1) Find local IP address, &\\
& neighbors, scan them to see & Discovery, & User-mode commands: & (2) Read ARP cache, & Conti,\\
Shares Hunter & which has Netbios/SMB & Lateral & ipconfig, arp, & (3) Scan hosts for & APT32\\
& sharing enabled, & Movement & nbtstat, net view & SMB/NetBIOS, &\\
& enumerate shares & & & (4) Enumerate network shares &\\
\hline
\end{tabular}}%
\label{tab:Laccolith profiles}
\end{center}
\end{table*}




Table \ref{tab:Test commands coverage} provides details on which commands of the emulation agent are involved in each profile, in order to get more insight about the adversary profiles of this experiment. In total, the profiles cover 7 commands implemented by the emulation agent, including actions to access the filesystem, the system registry, and to execute user-space commands. Moreover, the Laccolith agent provides additional commands for managing adversary emulation campaigns, not shown in the table for the sake of brevity. Overall, the newly implemented profiles allowed us to test the functionalities of Laccolith in depth.


To compare Laccolith to CALDERA, we performed the same experimental analysis for detectability. %In this case, as opposed to the campaign with CALDERA, Windows Defender is always active alongside the anti-virus under test.
Table~\ref{tab:Laccolith profile progress} shows the adversary profile execution progress for the four profiles against all the chosen AVs. % In addition, the results in this table also consider the injection phase, not just the progress of adversary profiles: if the injection fails, a profile will get a $0/N_{PA}$ score. \vittorio{Ha senso questa assunzione? In questo modo facciamo capire che lo score include sempre l'iniezione, come se questa avesse sempre successo, anche se in realtà andiamo a studiare la ''reliability'' dell'injection nella sezione successiva}
It is possible to notice that all profiles achieve complete execution progress, meaning that the AVs do not detect any of their actions.
%\marco{Kaspersky ormai è storia, l'injection funziona anche in presenza di Kaspersky; il fatto che c'è il crash dopo il dump di LSASS, invece, è ancora vero}
It is worth noting that the Shares Hunter profile has seven actions according to Table~\ref{tab:Laccolith profile progress}, instead of the four mentioned in Table~\ref{tab:Laccolith profiles}. This happens because this profile does not have an \textit{a priori} planning, but a dynamic one in which some actions depend on the outcome of the previous ones. In particular, since this profile performs network discovery operations, the result of its actions depends on whether there are any neighbors in the network. We assumed that the target VM interacted with the other VM recently, so it has the IP address of VM2 in its ARP cache alongside the gateway one. Both VM1 and VM2 have the NetBIOS sharing option active.
%Another thing to mention is that, after the dump of the LSASS process, the detach from the process makes the system crash, presumably because it is an invalid detach.



%\vittorio{Inserire figura che rappresenta setup di rete? Sì + spostare setup all'inizio della sezione in quanto è comune ad entrambe le analisi (CALDERA e Laccolith)}


\begin{table}[ht]
\centering
\caption{Coverage of commands of the Laccolith agent, with respect to the adversary profiles.}
\begin{center}
\resizebox{5cm}{!}{%
\begin{tabular}{ccc}
\hline
\textbf{Profile} & \textbf{Commands}\\
\hline
Thief & dir, read\\
\hline
Op-2 & write, setkey, version, dump\\
\hline
Ransomware & dir, read, write\\
\hline
Shares Hunter & read, usermode\\
\hline
\end{tabular}%
}
\label{tab:Test commands coverage}
\end{center}
\end{table}


\begin{table}[ht]
\centering
\caption{Adversary profile execution progress for Laccolith.}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\textbf{Profile} & \textbf{Windows Defender} & \textbf{Avast} & \textbf{AVG} & \textbf{Kaspersky} & \textbf{Avira}\\
\hline
Thief & \DrawPercentageBar{1} 3/3 & \DrawPercentageBar{1} 3/3 & \DrawPercentageBar{1} 3/3 & \DrawPercentageBar{1} 3/3 & \DrawPercentageBar{1} 3/3 \\
\hline
Op-2 & \DrawPercentageBar{1} 4/4 & \DrawPercentageBar{1} 4/4 & \DrawPercentageBar{1} 4/4 & \DrawPercentageBar{1} 4/4 & \DrawPercentageBar{1} 4/4 \\
\hline
Ransomware & \DrawPercentageBar{1} 5/5 & \DrawPercentageBar{1} 5/5 & \DrawPercentageBar{1} 5/5 & \DrawPercentageBar{1} 5/5 & \DrawPercentageBar{1} 5/5 \\
\hline
Shares Hunter & \DrawPercentageBar{1} 7/7 & \DrawPercentageBar{1} 7/7 & \DrawPercentageBar{1} 7/7 & \DrawPercentageBar{1} 7/7 & \DrawPercentageBar{1} 7/7 \\
\hline
\end{tabular}
%
}
\label{tab:Laccolith profile progress}
\end{center}
\end{table}



%The commands excluded from the profile coverage metrics were still tested, but in high-level actions, not fully-fledged operations. 

%\textcolor{red}{Questo paragrafo sembra troppo breve per stare in una sottosezione separata. Possiamo appendere alla sottosezione precedente.}


%\textcolor{red}{Bisognerebbe aggiungere un riferimento alla tabella, e spiegare brevemente come interpretarla (in particolare, spiegare il conteggio cumulativo), Serve ribadire quale è la conclusione: i 4 profili permettono di testare a fondo le funzionalità di Laccolith}



%\textcolor{red}{Sistemare reliability che diventa injection success}
The injection relies on overwriting the code of a system call or a kernel function called by a system call. Then, the shellcode executes only once, and the other concurrent calls return, as described in Section \ref{sec:injection process}. After loading the emulation agent, the original code is restored. This injection method can fail since the original code may be restored concurrently with a thread executing that function, which could encounter invalid opcodes due to misalignment or valid code that returns errors because of invalid values in the CPU registers. This failure results in an assertion failure (e.g., \textit{bug check}) within the kernel. Moreover, a critical system process (e.g., \textit{SYSTEM svchost.exe}) may crash because the system call does not exhibit the expected behavior.


%\textcolor{red}{Che significa "faulty"? Un bug nel nostro tool, oppure è un effetto inevitabile del nostro design?}

We performed preliminary experiments to gain insights into these events. In these initial experiments, we executed the injection after an increasing amount of time after the boot of the victim machine. We found that these events are more likely if the injection is performed within a few minutes right after the boot. If the injection is performed after a few minutes have passed since boot, the injection becomes more reliable. This behavior can be explained by the higher activity of system processes in the early phases of the start-up, which make high use of system calls and can expose these processes to failures. 
%After performing some tests \vittorio{fornire dettagli sui test? Test qualitativi eseguiti provando ad eseguire l'injection a distanza temporale sempre maggiore dal boot fino a verificare che l'injection falliva sempre meno volte}, we found that the probability of these events is higher in the first minutes after the boot; afterward, the injection becomes more reliable.



\begin{comment}

\begin{table*}[ht]
\centering
\caption{Empirical reliability of the injection technique.}
\begin{center}
\begin{tabular}{cccccc}
\hline
\textbf{Windows Defender} & \textbf{Avast} & \textbf{AVG} & \textbf{Kaspersky} & \textbf{Avira} & \textbf{Overall}\\
\hline
\DrawPercentageBar{0.95} 19/20 & \DrawPercentageBar{0.85} 17/20 & \DrawPercentageBar{0.85} 17/20 & \DrawPercentageBar{0.95} 19/20 & \DrawPercentageBar{0.90} 18/20 & \DrawPercentageBar{0.90} 90/100 90\% \\
\hline
\end{tabular}
\label{tab:Empirical reliability}
\end{center}
\end{table*}

\end{comment}

Therefore, the success of the injection method depends on the fraction of time the system spends executing the injected system call, and the percentage of cases that the system call is invoked by system processes. 
To quantify the effectiveness of the injection method, we performed more experiments by focusing on the favorable case of injection after boot has been completed, and the system has stabilized. 
The experiments consisted in repeating the injection method multiple times, each time from a clean condition (e.g., a full restart of the victim machine), and measuring how many times the injection was successful. 
%There are different approaches to studying the success probability of the injection method. The most precise one would be to leverage the knowledge about the possible failures and obtain the probability of success as the opposite of the probability of failure.
%The probability of failure is the sum of the probability of occurrence of the two failure events described in Section \ref{sec:injection reliability} if the failures are independent. An example of starting point to measure these probabilities is to measure the ratio at which the injected system call is called or the fraction of time the system spends executing that system call. It is not easy to estimate the exact probability of failure from there. A lower fraction of time does not automatically mean a lower probability of failure, because it could be a low fraction of time of critical processes as opposed to a higher fraction of time of common processes, which do not make the system reboot if they crash.
%Therefore, we preferred to perform a black-box empirical study, injecting the target multiple times and measuring how many times the injection was successful.
We conducted 20 experiments for each AV, re-booting the target VM each time to have independent samples. The timing of the injection was set to one minute after the Windows login prompt appeared. To verify if the injection was successful, we sent the agent an \textit{echo} and a \textit{close} command to check if it could execute commands and terminate gracefully. 
The injection fails if the connection is received, but it is impossible to perform these operations. If there is some minor error from user applications, which cannot be attributable to a security alarm (e.g., a generic ``unknown exception in explorer.exe''), we still consider the injection successful.

Table~\ref{tab:Empirical reliability} summarizes the experimental results. The AV does not impact the injection success since all the setups with the different AVs exhibit similar behavior. The overall success rate of the injection method has been $90/100$, hence 90\% of experiments. 
Considering a margin of error of $1/\sqrt{N}$, where $N$ is the overall number of repetitions \cite{42}, the success rate of the injection method ranges between 80\% and 100\%. Even in the worst case, the success rate is still higher than the probability of running CALDERA and Inceptor without being detected, which had approximately a 25\% probability of success, neglecting the issue of bypassing UAC which makes the process even more uncertain.

It is worth noting that the injection success for Laccolith can be further improved by injecting into a target linear region of code that is executed less frequently, in order to reduce the probability that the injection clashes with the execution of the target system call. This can be achieved by a preliminary profiling of the execution frequency of system calls. Since the profiling depends on the workload of the specific system under evaluation, and since this represents an engineering problem, we consider this beyond the scope of our research work. 
%\vittorio{Aggiungere frase su "possibilità di profilare system call per capire quali soon meno chiamate e trovarne una che viene chiamata di meno e può avere probabilità più alta di successo"}
%\marco{Questo paragrafo si basa sul fatto che il paragrafo "Selection of AV/EDR Solutions" sia stato scritto, perché sopra c'è scritto "20 experiments for each AV", quindi il numero N di ripetizioni citato in questo paragrafo è 20 * 5 = 100, però questa cosa non può essere chiara se non si specificano quali sono gli AV. Inoltre, visto che stiamo parlando di "overall probability", N lo definirei come "overall number of repetitions".}

\begin{table}[ht]
\centering
\caption{Injection success for Laccolith.}
\begin{center}
\resizebox{5cm}{!}{%
\begin{tabular}{cc}
\toprule
\textbf{Anti-virus} & \textbf{Injection Success} \\
\toprule
Windows Defender & \DrawPercentageBar{0.95} \hspace{2pt} 19/20 \\
\hline
Avast & \DrawPercentageBar{0.85} \hspace{2pt} 17/20 \\
\hline
AVG & \DrawPercentageBar{0.85} \hspace{2pt} 17/20 \\
\hline
Kaspersky & \DrawPercentageBar{0.95} \hspace{2pt} 19/20 \\
\hline
Avira & \DrawPercentageBar{0.90} \hspace{2pt} 18/20 \\
\hline
\hline
Overall & \DrawPercentageBar{0.90} 90/100 \\
\bottomrule
\end{tabular}%
}
\label{tab:Empirical reliability}
\end{center}
\end{table}



==> tex/old/introduction.tex <==
\label{sec:introduction}
%Cyber-attacks have become a severe threat in several domains where the impact can be exceedingly high (e.g., in terms of service outages, private data breaches, and intellectual property theft), such as healthcare, manufacturing, telecom, energy, and transportation. Modern attacks are very challenging, as they evolved into \emph{Advanced Persistent Threats} (APTs) from cybercriminal and state-sponsored groups. In APT, attackers accomplish their goals through a carefully-planned sequence of malicious actions, which are performed over a long time, while being careful to stay undetected. Well-known examples include the Stuxnet attack, which has been sabotaging Iran's nuclear centrifuges since 2005 and was uncovered in 2010 \cite{StuxnetDossier}, GhostNet \cite{GhostNet}, and Carbanak \cite{Carbanak}. The time an APT attack goes undetected (``dwell time'') has been estimated to be up to hundreds of days \cite{MandiantTrends}.
\emph{Advanced Persistent Threats} (APTs) have become a severe threat in several domains where the impact can be exceedingly high (e.g., in terms of service outages, private data breaches, and intellectual property theft), such as healthcare, manufacturing, telecom, energy, and transportation. In APT, attackers accomplish their goals through a carefully-planned sequence of malicious actions performed while being careful to stay undetected. These attacks are getting even more challenging to counter, as they are carried out by cybercriminal and state-sponsored groups. 
Well-known examples include the Stuxnet attack, which has been sabotaging Iran's nuclear centrifuges since 2005 and was uncovered in 2010 \cite{StuxnetDossier}, GhostNet \cite{GhostNet}, and Carbanak \cite{Carbanak}. The time an APT attack goes undetected (``dwell time'') has been estimated to be up to 700 days \cite{MandiantTrends}. With all this time to act, APTs can cause irreparable damage.

%https://www.mandiant.com/resources/m-trends-2021
%https://citizenlab.ca/wp-content/uploads/2017/05/ghostnet.pdf
%https://media.kasperskycontenthub.com/wp-content/uploads/sites/43/2018/03/08064518/Carbanak_APT_eng.pdf

\emph{Adversary emulation} is the most effective prevention against APTs \cite{Applebaum2016IntelligentAR}. Adversary emulation is a proactive approach that reproduces the actions of an APT inside a target computer infrastructure. It grants several advantages for security training and assessment purposes, such as understanding threats, realistic and comprehensive testing, identification of weaknesses, and validation of security controls. This approach focuses on post-compromise scenarios, assuming that the APT has already gained access to the target infrastructure and is infecting hosts and devices silently, escalating privileges, and exfiltrating data. Adversary emulation is usually exercised in virtualized environments (\emph{cyber-ranges}) and, in general, it encompasses time-consuming activities that engage human personnel (\emph{red teams}). 
Several tools aim to automate adversary emulation \cite{zilberman2020sok}, which offer automated procedures that implement APT techniques, as learned from threat intelligence sources. These tools typically automate actions for information gathering, lateral movement across hosts, connections to command-and-control servers, and privilege escalation. 

A fundamental characteristic of APTs is the adoption of \emph{anti-detection} techniques, to hide their traces from AV (anti-virus) products and EDR (endpoint detection and response), a modern evolution of AVs, and to persist in the target infrastructure as long as possible. 
Therefore, adversary emulation also needs to apply anti-detection techniques, in order to perform realistic and fruitful security assessments and training activities. Examples of anti-detection techniques include un-hooking probes used by EDRs to instrument and monitor DLL and API uses \cite{HookingMemoryProtection}; disabling or hampering event tracers, such as the Event Tracing for Windows (ETW) subsystem \cite{ETWbypass}; using malicious kernel modules to hide processes and files \cite{Outflank}; obfuscating malicious payloads (e.g., shellcodes) \cite{EvadingShellcode, EDRShellcode}. 
However, it is challenging for adversary emulation tools to automate anti-detection techniques, since both APTs and AV solutions are continuously evolving, in a ``cat-and-mouse'' game. 
%Examples of anti-detection techniques include un-hooking probes used by EDRs to instrument and monitor DLL and API uses \cite{HookingMemoryProtection}; disabling or hampering event tracers, such as the Event Tracing for Windows (ETW) subsystem \cite{ETWbypass}; using malicious kernel modules to hide processes and files \cite{Outflank}; obfuscating malicious payloads (e.g., shellcodes) \cite{EvadingShellcode, EDRShellcode}. 
%Automating these techniques is problematic since AV/EDR solutions are continuously developed to respond to anti-detection techniques, in a ``cat-and-mouse'' game. 
Currently, adversary emulation tools have to be customized for the specific AV/EDR to evade, which requires considerable skills and development efforts \cite{iRedTeam, Cyberstruggle}, and is prone to become outdated and ineffective. For these reasons, emulating anti-detection techniques in automated ways in adversary simulations is still impractical. This is a significant limitation in realistically emulating APTs.
%In this work, we present an experimental analysis on the issue of anti-detection in adversary emulation, and we introduce a novel solution for adversary emulation with anti-detection capabilities. 

In this work, we investigate a novel solution for adversary emulation with anti-detection capabilities, to avoid the previously mentioned ``cat-and-mouse'' game. We tested state-of-the-art solutions for adversary emulation (\emph{MITRE CALDERA} \cite{zilberman2020sok}) and for anti-detection (\emph{Inceptor} \cite{Inceptor}) against multiple AV/EDR products. We found that several malicious actions (and even the installation of the emulation agent) cannot evade detection, thus limiting the realism of emulated attacks. Laccolith is based on a novel \emph{hypervisor-based} architecture for adversary emulation. This design choice was led by the fact that cybersecurity exercises typically happen in virtualized environments \cite{yamin2020cyber, beuran2018integrated, vceleda2015kypo, wroclawski2016deterlab, ferguson2014national}. 

Our solution (\emph{Laccolith}) enables the non-detectable execution of malicious actions, by injecting them from the lowest layers of the software stack. We experimented with Laccolith against several AV solutions for Microsoft Windows. The results showed that Laccolith was able to execute all of the malicious actions, which evaded all of the tested AV products. Our solution does not require customizations for the specific version of the target system, as it can reliably execute non-detectable actions across different versions of the guest OS and AV products. %For the sake of clarity, AV evolved into EDR products over time, which are more sophisticated solutions that offer additional features, such as centralized management. In the following, we will use the term AV with an extended meaning to refer to both kinds of solutions.

%\textcolor{red}{Chiarire che AV si soon evoluti in EDR (più sofisticati) e che usiamo AV come terminologia "estesa"}

The remainder of the paper is structured as follows. In Section \ref{sec:background}, we elaborate on background concepts about APTs and adversary emulation. In Section \ref{sec:solution}, we present the proposed solution for adversary emulation. In Section \ref{sec:experiment}, we illustrate experiments on the anti-detection of existing solutions and our proposed one. In Section \ref{sec:related}, we discuss related work. Section \ref{sec:conclusion} concludes the paper.

==> tex/old/related.tex <==
\section{Related Work}
\label{sec:related}

\input{tex/table}

Zilberman \emph{et al.} \cite{zilberman2020sok} analyze and classify several adversary emulators. The authors defined a set of criteria and a methodology to evaluate the threat emulators; a taxonomy of the qualities of the threat emulators; and guidelines for choosing an appropriate adversary emulator, given the specific environment and the security assessment tasks. Among the criteria defined in this work are OS compatibility, changes needed in the security array, ATT\&CK TTPs coverage, procedures configuration, and required security expertise.
In this section, we further analyze and discuss the most popular and mature adversary emulation tools according to the survey \cite{zilberman2020sok}.
%\textcolor{red}{Possiamo forse concludere il paragrafo precedente, dicendo che in questa sezione approfondiamo i tool più maturi/diffusi/... in base a quel survey.}

\emph{Atomic Red Team} \cite{AtomicRedTeam} is a library of scripts to emulate adversary behavior. Every script implements a single ATT\&CK technique or sub-technique (277 out of 719, 231 out of 507 for Windows). It can be used for specific/atomic tests but is not suitable to emulate complex scenarios.
\emph{Red Team Automation} \cite{RedTeamAutomation} is a script framework that implements single techniques from the ATT\&CK framework (around 50) for security assessment purposes. It does not offer built-in scripts for multi-procedure attacks. 
\emph{APTSimulator} \cite{APTSimulator} is a batch script-based tool for Windows that offers around 30 attack techniques to emulate post-compromise scenarios. These techniques leverage external tools such as Mimikatz and PowerSploit. 
\emph{Infection Monkey} \cite{InfectionMonkey} is an adversary emulation tool composed of two main elements, the server (Monkey Island) and the agents (Monkeys). Infection Monkey implements a few ATT\&CK techniques, mostly for Initial Access and Lateral Movement. As CALDERA, Infection Monkey does not offer any anti-detection capability to hide malicious actions, and AVs easily detect its agents' activities \cite{zilberman2020sok}. 
\emph{Metta} \cite{Metta} is an adversary emulator developed by Uber Technologies to assess endpoint security. It provides techniques for various tactics, such as Discovery, Credential Access, and Defense Evasion. However, it does not emulate complete attacks but focuses on the assessment of specific targets. 
\emph{DumpsterFire} \cite{DumpsterFire} offers a collection of actions (fires) that can be chained together into complex attacks (dumpster fires). Fires are not based on ATT\&CK framework techniques and are organized into categories: Network Scans, File Downloads, Websurfing, Account Bruteforcing, Filesystem Activities, Malware, Custom OS Commands, and Shenanigans. It can only execute on Linux.
\emph{Invoke-Adversary} \cite{InvokeAdversary} is a PowerShell script to test security mechanisms. It offers 39 techniques grouped by ATT\&CK tactics. It does not offer multi-procedure scripts and does not support Lateral Movement. Moreover, its procedures are usually detected by AVs, making it not suitable for usage in real-world scenarios.
\emph{Sliver} \cite{Sliver} is a C2 framework for adversary emulation. It offers multi-platform agents that communicate with the C2 server using different protocols (e.g., HTTP, DNS, Mutual TLS). It also provides attacker capabilities through plugins called armories. Sliver does not offer any AV-evasion capability as explicitly stated in its documentation. 

Table~\ref{tab:Tools comparison} summarizes the comparison among the mentioned adversary emulation solutions. It is possible to notice how the tools that provide an advanced architecture with a C2 server (i.e., CALDERA, Infection Monkey, and Sliver) need to install an agent on the target system. None of the other tools, which do not use an agent, offer command-and-control capabilities. In terms of ATT\&CK tactics coverage, Atomic Red Team is the best-performing tool, covering 11 tactics. CALDERA has a similar coverage to Atomic Red Team and is the most complete among the C2 frameworks. CALDERA does not cover Initial Access, because it is not relevant in adversary emulation, and the Impact tactic, unlike our solution which encompasses it in the Ransomware profile. 
Moreover, CALDERA surpasses the other C2 frameworks regarding complex attacks, providing built-in attacks and capabilities to develop custom ones. CALDERA also provides a plugin to leverage Atomic Red Team tactics and techniques, making it the best-performing tool among the existing ones. It is worth noting that none of the analyzed tools provide anti-detection techniques to evade AV/EDR products.

Our proposed solution differs from the previous ones. Laccolith represents a C2 framework that does not need to explicitly install an agent on the victim machine, unlike CALDERA, Infection Monkey, and Sliver. It also offers profiles based on real-world APTs and mapped to the ATT\&CK matrix,  covering the same tactics of Atomic Red Team. Most importantly, Laccolith enables the emulation of malicious actions without being detected by AV and EDR solutions. Moreover, it is portable across different versions of the target guest OS and does not require any customization related to the specific AV/EDR. To achieve all these abilities, Laccolith leverages virtualization, widely used in infrastructures for cybersecurity exercises, as illustrated in the following.

Yamin \emph{et al.} \cite{yamin2020cyber} performed a literature review on Cyber Range platforms and security testbeds, highlighting that most solutions leverage virtualization to set up security training and assessment environments. The use of virtualization spans multiple domains, such as Internet-of-Things (IoT), autonomous systems, SCADA systems, and critical infrastructures.
Beuran \emph{et al.} \cite{beuran2018integrated} proposed \emph{CyTrONE}, a framework for cybersecurity training. CyTrONE is equipped with a Learning Management System (LMS) for the trainees and offers a Cyber Range that relies on virtualization technologies. The Cyber Range is instantiated using a variable number of VMs, depending on the specific training scenario.
\emph{KYPO} \cite{vceleda2015kypo} is a platform for cyber defense exercises developed by Masaryk University. It aims to emulate attacks on critical infrastructures in a controlled environment. For this purpose, KYPO leverages cloud computing technologies (e.g., OpenStack), and relies on virtualization for hosts and networks.
\emph{DETERlab} \cite{wroclawski2016deterlab} is a solution for cybersecurity experimentation developed in the context of the \emph{DETER} project. It provides a flexible and realistic environment for security training and assessment. These goals are fulfilled by leveraging virtualization technologies, which enable easy reconfiguration and scalability. 
The \emph{National Cyber Range} (NCR) \cite{ferguson2014national} is a facility for cybersecurity testing established by the Defense Advanced Research Projects Agency (DARPA). Its purpose is to provide an environment to design and test new ways to respond to the most recent threat actors. The range combines physical and virtualized resources and networks according to the nature of the simulation. 


%\textcolor{red}{Spiegare brevemente perchè due tactics non sono coperte da CALDERA (initial access, impact), forse perché initial access non è di interesse per adversary emulation, e che noi compensiamo Impact nella nostra analisi aggiungendo il profilo Ransomware.}

==> tex/old/solution.tex <==
\section{Proposed solution}
\label{sec:solution}

In this section, we present our proposed solution for adversary emulation with anti-detection. We first provide an overview, including our system model and assumptions for our design. We then describe in detail the proposed design. Finally, we provide information about our implementation. 

\subsection{Overview}
\label{sec:overview}
We based the design of Laccolith on a set of assumptions applied in general for adversary emulation. The assumptions include:

\begin{itemize}
    \item Adversary emulation focuses on post-compromise scenarios where the attacker has already gained a foothold inside the system (e.g., through phishing or exploiting a vulnerability) and is performing more malicious actions, such as gaining more privileges and stealing information.
    \item Adversary emulation is performed in the context of cybersecurity exercises, which are authorized and overseen by a ``white team'' in the organization (e.g., system administrators). Adversary emulation can be warranted system privileges as needed.
    \item Laccolith is designed to perform adversary emulation in a virtualized environment, where hosts are deployed using virtual machines. This is typically the case in cybersecurity exercises, where dedicated networks and hosts are deployed using virtualization infrastructures \cite{beuran2018integrated, schoonover2018galaxy, kouril2014cloud}. For example, all the most popular Cyber Ranges run in the cloud, leveraging virtualization technologies \cite{yamin2020cyber, ferguson2014national, vceleda2015kypo}. Moreover, the solution applies to organizations that run their own private data centers, which is often the case for high-criticality domains such as defense, critical infrastructures, and healthcare \cite{dhaya2021dynamic, regola2013storing}. Instead, the proposed solution is not meant for networks and services running on bare-metal hardware.
    \item Endpoints in the environment can be equipped with AV products, as in the case of real computer networks. This assumption is not met by traditional adversary emulation tools, which require turning off AV products to install and run the tools \cite{zilberman2020sok}. Laccolith is designed to overcome this limitation.
\end{itemize}

The driving idea for our design is to leverage kernel- and hypervisor-level privileges to execute malicious actions, which would otherwise be detected if performed from user level (i.e., from an application process).\footnote{The name \emph{Laccolith} reflects the injection of malicious actions from the lower layers of the software stack. A laccolith is a volcanic phenomenon where magma rises through the Earth's crust, forcing rock strata upward.}
AV solutions typically use ``hook'' functions to intercept invocations of the system calls. When applications (including malicious ones) invoke system calls, the hook functions are executed instead (e.g., by replacing pointers in the system call table), which can check the invocation and detect suspicious activities. In traditional adversary emulation (Figure \ref{fig:Adversary Emulation architecture}), an agent process executes malicious actions on behalf of a red team by issuing system calls that access OS resources, such as files, processes, connections, and others.
Without any anti-detection technique, AV products can detect these actions by checking system calls.

\begin{comment}
    - Security checks basati su: system call hook ecc
    Specificare questi requisiti e poi spiegare che senza tecniche di anti-detection AE tradizional viene rilevata facilmente ecc
    - Di conseguenza spiegare perché la scelta della soluzione basata su hypervisor: perché inteso nell'ottica di "perché la soluzione hypervisor-based permette di risolvere questo problema"
\end{comment}

To perform non-detectable actions, it is necessary to use system calls not monitored by the AVs, hence from the kernel level. Consequently, the hypervisor level is the ideal choice to accomplish that, leveraging virtual machine introspection (VMI) techniques. In our design, we circumvent the anti-virus checks by introducing an emulation agent from the hypervisor. Since the hypervisor has full privileges on a physical machine, it can warrant full read and write access to the state of a virtual machine. We use these privileges to install an emulator into the kernel of the guest OS of the virtual machine. This way, it is possible to directly access guest memory, without issuing user-space system calls. From the agent installed in the guest OS kernel, we can perform malicious actions by calling kernel-level APIs. Such calls cannot be detected by AV products since they are not subject to security checks.

Moreover, we designed the kernel-level agent with the ability to run user-level commands, as in traditional adversary emulation tools. Therefore, red teams can combine kernel-level and user-level actions to perform both detectable and non-detectable actions. This flexibility enables red teams to perform realistic training exercises for security teams, where the emulated APT leaves only a few selected traces of malicious activity.

\begin{figure}[!htbp]
\centering
\centerline{\includegraphics[width=\linewidth]{img/Laccolith Architecture.png}}
\caption{Laccolith architecture.}
\label{fig:Laccolith architecture}
\end{figure}

%\hl{NOTA: La figura andrebbe aggiornata per indicare "emulation agent", "emulation server", ed "emulation manager" (fuori dallo hypervisor). È meglio utilizzare lo stesso stile di figura 1, eventualmente con dei grigi invece che colori.}

%In addition to the emulation agent, Laccolith comes with additional components for managing adversary emulation. As in existing adversary emulation tools, a central \emph{emulation manager} orchestrates emulation agents across the network, and issues actions to be executed on the victim hosts. Therefore, the red team controls the emulation agents to reproduce the actions of an APT campaign. The red team can interact with the emulation manager through web and command-line interfaces.
Laccolith offers a complete architecture for adversary emulation: a central \emph{emulation manager} orchestrates \emph{emulation agents} across the network and issues actions to execute on the victim hosts. Therefore, the red team controls the emulation agents to reproduce the actions of an APT campaign. The red team can interact with the emulation manager through web and command-line interfaces.
%At the same time, security personnel (``blue teams'') aims to...

On each physical machine, Laccolith installs an \emph{emulation server}, which runs at hypervisor-level, and manages the emulation agents on each physical machine. The emulation server installs the emulation agents on each virtual machine by leveraging VM introspection techniques to modify guest memory and create a new execution flow inside the guest kernel. 
Moreover, the emulation server forwards communication between the emulation agents and the manager. The communication traffic between the components of Laccolith is invisible to the participants of the cybersecurity exercise since this traffic flows at the physical level, beyond the virtual networks of the virtual machines.



\begin{comment}
\subsubsection{Injection}
\label{sec:injection}
The injection of the high-privileged agent must be performed using the privilege of the hypervisor.

The injection should leverage full read/write (R/W) access to the RAM of the victim VM in real-time, like an attacker that was able to gain access after a successful exploit. In addition to that, since the hypervisor is external to VM-specific page mechanisms, it has R/W access bypassing page permissions.

This post-exploitation phase can also be simulated with the help of virtual machine introspection (VMI) techniques, for example, with Volatility \cite{Volatility}. This is necessary to have visibility of kernel symbols of the target VM.

After the successful injection of the agent, the VM must be able to continue its operations, that is, it must not crash.


\subsubsection{Agent}
\label{sec:agent}
The injected agent must have defense evasion capabilities, effective against common AV/EDR solutions. Therefore, it must run with high privilege, ideally in kernel space.

It must connect to a C2 server and be ready to execute the commands it receives and provide feedback about their outcome. The agent also needs to implement a set of commands complex enough to allow the emulation of adversary profiles.

Once the campaign is completed, the agent should terminate gracefully, without making the system crash: this will happen when the C2 server sends a 'close' command to the agent itself.

In addition to that, it would be better if the agent was able to execute actions both in a stealth way and in a less stealth way, to offer the possibility of configuring the evasion capabilities as needed. This is necessary to make a specified set of activities easier to detect during a purple team engagement.

\subsubsection{Framework}
\label{sec:framework}
The proposed solution should come with a complete framework to orchestrate the injection and execution of malicious actions. 
First, it must automate injection, using the access to VM RAM and with the help of VMI techniques, as mentioned in Section \ref{sec:injection}. The injection automation subsystem must be capable of modifying the run-time parameters of the injected payloads. In addition to that, it must be able to automatically detect the available domains (the terms VM and domain will be used interchangeably) to inject, and it should be decoupled from the underlying virtualization technology.

Second, the framework needs to implement a C2 server to receive connections, store information about them and make them available, handle multiple connections concurrently (like Metasploit, a penetration testing framework also used for adversary emulation \cite{Metasploit}), and be able to conduct complex sequences of commands automatically (like Caldera’s \textit{Autonomous red-team engagements} \cite{CALDERAdocs}).

Third, it needs to offer one or more interfaces to handle:
\begin{itemize}
    \item Injection of domains;
    \item Access to C2 functions, such as listing received connections, sending a command to an agent, reading the output of a command, and starting an autonomous operation;
    \item Customization of some parameters, for example, choosing which payload to inject;
    \item Basic file upload and download functions: the upload can be useful for custom operations, whereas the download is useful for exfiltrated files.
\end{itemize}

These functions can be split into more than one interface, with the idea that some functions can be more user-friendly in another type of interface rather than making all of them fit together in a unique interface.

Fourth, it should be easy to deploy and customize.
\end{comment}


\subsection{Emulation server}
\label{sec:emulation_server}
The \textit{emulation server} is the trickiest component in our architecture. It is responsible for injecting \textit{emulation agents} inside the VMs, by leveraging read/write (R/W) access permissions to modify their state. It relies on installing a kernel-level agent to avoid detection from AV products.


%It does not rely on installing a user-level process in the VM since it would trigger detection by AV products. \vittorio{Non diciamo cosa non fa ma cosa fa}

%\textcolor{red}{Far capire al lettore perché sono necessari gli step descritti in 3.2.1, spiegare che gli indirizzi virtuali non sono noti e quindi serve workaround dell'egg ecc, perché bisogna scrivere due pezzi di codice e non uno (riprendere spiegazioni tesi di Marco a riguardo). Parte della complessità è dovuta al fatto che bisogna scoprire che una porzione di memoria user space (freccia 7) sia libera e che l'allocatore del kernel sia occupata}

\subsubsection{Overview of the injection method}
\label{sec:injection process}

The emulation agent needs to run in a dedicated area of the virtual memory of the VM. However, the allocation of virtual memory cannot be directly performed from the hypervisor but needs to be performed by the guest OS kernel, which is aware of the current layout of memory allocations. Consequently, the injection of the emulation agent consists of two stages. 
The first stage consists of the injection of a small program (a ``shellcode'') in kernel space, responsible for allocating the code region for the emulation agent, while the second stage entails bootstrapping the asynchronous execution of the agent in that area. The injector overwrites a piece of existing kernel code with the shellcode to make it executed by the kernel. Differently from the \emph{injector} (which runs in the hypervisor and can only work with ``guest physical'' memory addresses), the shellcode can allocate and access the ``guest virtual'' memory addresses since it runs within the guest OS kernel.
Before selecting the target kernel code to overwrite, we need to address two requirements for the shellcode:
\begin{enumerate}
    \item \textit{Space}: the shellcode should be small enough to fit into the target kernel code;
    \item \textit{Behavior}: if the overwritten kernel code is invoked, the shellcode needs to handle the call without hanging the calling process. Moreover, it should also handle the case of concurrent calls from different processes.
\end{enumerate}

We consider the code of system calls for the injection of the shellcode since their position in the virtual memory of the VM can be identified with \emph{virtual machine introspection} (VMI) techniques. VMI is an approach to gain visibility and control over VMs without modifying the guest OS \cite{garfinkel2003virtual}. 
Moreover, system calls are regularly invoked by applications, thus assuring that the shellcode will be eventually executed. 
The previously mentioned requirements are the reason why we cannot trivially overwrite a system call with the code of the \emph{emulation agent}: the first one would restrict the size of the agent, which would hamper the implementation of malicious actions; the second requirement implies that the system call code needs to be restored at some point, thus removing the injected code. %Therefore, we split the injection method into two stages, by first loading a \emph{shellcode} that meets these constraints; then, the shellcode is responsible for allocating the code region for the emulation agent and for bootstrapping the asynchronous execution of the agent in that area. Differently from the \emph{injector} (which runs in the hypervisor and can only work with ``guest physical'' memory addresses), the shellcode can allocate and access the ``guest virtual'' memory addresses since it runs within the guest OS kernel.

%We consider the code of system calls for the injection of the shellcode since their position in the virtual memory of the VM can be identified with \emph{virtual machine introspection} (VMI) techniques. VMI is an approach to gain visibility and control over VMs without modifying the guest OS \cite{garfinkel2003virtual}. 
%Moreover, system calls are regularly invoked by applications, thus assuring that the shellcode will be eventually executed. 
%Before selecting the target system call to overwrite, we need to address two requirements \vittorio{sono requirements, bisogna spostarlo sopra quando si parla di shellcode} for the shellcode:
%\begin{enumerate}
%    \item \textit{Space}: The shellcode should be small enough to fit into the system call code;
%    \item \textit{Behavior}: It needs to exit gracefully without hanging since user-space processes expect the system call to return quickly after the invocation. Moreover, it should handle the case of being called multiple times by concurrent processes. \vittorio{Spiegare bene che il comportamento deve essere r}
%\end{enumerate}
%These requirements are the reason why we cannot trivially overwrite a system call with the code of the \emph{emulation agent}: the first one would restrict the size of the agent, which would hamper the implementation of malicious actions; the second requirement implies that the system call code needs to be restored at some point, thus removing the injected code. Therefore, we split the injection method into two stages, by first loading a \emph{shellcode} that meets these constraints; then, the shellcode is responsible for allocating the code region for the emulation agent and for bootstrapping the asynchronous execution of the agent in that area. Differently from the \emph{injector} (which runs in the hypervisor and can only work with ``guest physical'' memory addresses), the shellcode can allocate and access the ``guest virtual'' memory addresses since it runs within the guest OS kernel.

%which overwrites the system call but will be responsible for the allocation of the code region for the agent and the asynchronous execution of the agent in that area.
%The injection process can be divided into two stages: first-stage injection of the \emph{shellcode}, then second-stage injection of the \emph{emulation agent} itself. The complete process is shown in Figure \ref{fig:Injection Chain}. 
%The first step is finding an injection point for the shellcode, which is responsible for allocating the code region for the emulation agent and the asynchronous execution of the agent in that area. 
%System calls are a good fit as injection points because they are eventually invoked by system processes. 
To choose a target system call to overwrite, we look for a \textit{linear region of code}, i.e., a memory region that meets the following requirements:
\begin{enumerate}
    \item The memory region is from the code area of the guest OS kernel; this code is only executed by starting from the initial address of the memory region. For example, this requirement is satisfied if the memory region exactly matches the code of an individual kernel function; in this case, other kernel code only jumps to the initial address of the memory region (i.e., there are no jumps to addresses in the middle of the memory region).
    \item The code in the memory region does not call other functions. This requirement avoids that code not belonging to the memory region returns in the middle of the region.
    \item The region fits inside a memory page without crossing page boundaries.
\end{enumerate}

The first and second requirements allow us to inject arbitrary code in the memory region without risking the kernel jumping in the middle of the region, which would likely raise CPU exceptions (e.g., executing an invalid opcode). The shellcode will execute when the kernel executes the memory region, in place of the original code. 
The third requirement is necessary to make it easier to modify the VM memory from the hypervisor since code over multiple pages in virtual memory does not necessarily map to contiguous pages in physical memory. 
An example of an eligible memory region in Microsoft Windows OS is the \textit{MmQueryVirtualMemory} function (about $3,800$ bytes), which is called by the \textit{NtQueryVirtualMemory} system call. In general, linear regions of code are plentiful and easy to find: given the function call graph of the kernel code (e.g., \textit{ntoskrnl.exe} in Microsoft Windows), a linear region of code is a function without fan-out that fits within a single memory page. %For example, if we consider \textit{ntoskrnl.exe}, i.e., Windows kernel, it is easy to check if a region of code is linear, since ntoskrnl starts from an address aligned with page boundaries. 
%\vittorio{Spiegare se linear regions sono abbondanti e facili da trovare, in modo da chiarire se l'approccio è effettivamente portable su altre versioni/altri OS}


\subsubsection{Injection method}
\label{sec:detailed injection}

\begin{figure*}[!htbp]
\centering
\centerline{\includegraphics[width=\textwidth]{img/Injection Chain.png}}
\caption{Injection method in Laccolith.}
\label{fig:Injection Chain}
\end{figure*}


%\textcolor{red}{Descrivere cosa ci aspettiamo di ottenere con VMI (quali info): processor di virtual address to physical address}
The injection method is shown in Figure \ref{fig:Injection Chain} and summarized as follows. First, the \emph{injector} searches the code of the target system call in memory (step \circled{1}). Since the \emph{injector} can only access VM memory through guest physical addresses, it scans memory by looking for code that matches the initial unique bytes of the target system call. The injector leverages VMI to make this process more portable and efficient: it determines from VMI the unique bytes of the system call from the kernel binary, and the relative offset of the system call within the kernel virtual address space. Then, it only scans memory pages on that relative offset. 
Once the position of the target system call has been found, the \emph{injector} overwrites it with the shellcode (step \circled{2}). 

Then, the shellcode will eventually execute when the system call is invoked. 
The shellcode will execute for a limited time, long enough to allocate a memory area and communicate to the emulation server that the memory area is ready for loading the emulation agent (the last step of the method). 
The shellcode uses the APIs of the guest OS kernel (step \circled{3}) to allocate a contiguous area of guest virtual memory (for example, the \textit{MmAllocateContiguousMemory} function from the Windows Driver Kit (WDK) \cite{22}). 
The shellcode then obtains pages of contiguous virtual memory (e.g., $16$KB in our implementation) from the guest virtual address space (step \circled{4}), without the constraints that previously applied for the shellcode. 

During this time window, any other concurrent call to the target system call must immediately return, since the shellcode should execute only once. For this purpose, the shellcode acquires a spinlock in a \emph{non-blocking} way, without busy-waiting if the spinlock is already held (e.g., using the \textit{xchg} instruction on Intel architectures \cite{31}). Once acquired, the shellcode holds the spinlock to avoid concurrent executions.

Next, the shellcode writes a pre-defined value (``egg''), also known by the injector, within the allocated memory area. This way, the injector can find the allocated memory area using only guest physical addresses. %\textcolor{red}{This cookie is called \textit{egg} because the injector must search it and overwrite it with the second-stage shellcode, which is bigger, so 'the egg hatches'. (spiegare che lo shellcode alloca 16 KB di memoria contigua in cui scrive l'egg per segnalare che è occupata (e segnalare all'injector che deve scrivere lì)}
The injector overwrites the allocated memory with the code of the emulation agent (step \circled{5}). Finally, the shellcode sets up an execution context to run the emulation agent in the kernel. Again, the shellcode uses APIs of the guest OS kernel to create a kernel thread (step \circled{6}), such as using the \textit{PsCreateSystemThread} function in Windows. The new kernel thread will be configured to run the code of the emulation agent in the allocated memory area (step \circled{7}), e.g., using the \textit{StartRoutine} of the Windows kernel. As a result, the emulation agent will execute with high privileges since it will run in kernel mode. After the agent starts, the injector restores the original system call code to leave no traces in the target VM other than the emulation agent (step \circled{8}).
%this is accomplished by creating a kernel thread that executes the emulation agent code (step \circled{6}). Consequently, the emulation agent will have high privileges since it will run in kernel mode (step \circled{7}). After the agent starts, the injector restores the original system call code to leave no traces in the target VM other than the agent itself (step \circled{8}).
%Once the target system call has been chosen and its address has been retrieved (step \circled{1}), the \emph{injector} will overwrite it with the shellcode (step \circled{2}) for a limited time, long enough to communicate to the emulation server that the memory area for the injection of the emulation agent is ready. During this time window, any other concurrent call to the target system call will immediately return. Then, the shellcode will be eventually executed, when the system is called, and it will allocate the memory area for the emulation agent, writing a specific value (''egg'') in it (step \circled{3}, \circled{4}). Next, the injector looks for the egg and, after it is found, overwrites it with the emulation agent code (step \circled{5}). The emulation agent needs an execution context to run in the kernel: this is accomplished by creating a kernel thread that executes the emulation agent code (step \circled{6}). Consequently, the emulation agent will have high privileges, since it is running in kernel mode (step \circled{7}). After the agent is started, the original system call code is restored to leave no traces in the target VM other than the agent itself (step \circled{8}).

%Lo emulation server è il componente più critico e complesso della nostra soluzione. Si occupa di accedere alla memoria delle VM per installare lo emulation agent, utilizzando solamente i permessi di accesso in lettura e scrittura alla memoria. Non può fare affidamento sulla installazione di un processo in user-level, che triggererebbe la detection.

%Spiegare il procedimento di injection. Puoi eventualmente dividere la discussione in sotto-sotto-sezioni. Evidenziare che il risultato finale è che il codice dell'emulation agent è nella memoria del guest, e che esiste un flusso di esecuzione (thread) che esegue il codice dello agent a livello kernel, con i privilegi del guest OS. Dopo l'iniezione non sono presenti altre tracce residue nel guest.

%Through Volatility, we were able to get the virtual addresses of the system call to inject the first stage shellcode. The virtual address was not sufficient to perform the injection, since our injector can only write the RAM's live image using the offsets of physical addresses. To fill this \textit{semantic gap}, we implemented a function to retrieve the corresponding physical address for a given virtual address, based on the assumption that, if we consider a sufficient number of bits of the system call address, it is likely to be a unique sequence \cite{17}.



\subsection{Emulation agent}
\label{sec:emulation_agent}

The \textit{emulation agent} is responsible for receiving and executing commands from the emulation server. Since it runs with high privileges, it can call kernel APIs as if it were a kernel module. The agent can also access the OS resources, such as the process descriptors and the system registry. Through these resources, the agent can access the memory of user-level processes since a process descriptor indicates the memory regions where the code and data of a process are. It can both read (e.g., process dumping to steal passwords, tokens, and other data) or write (e.g., process/DLL injection to hide malicious code in system processes) the processes' memory, and modify the system configuration, e.g., changing the registry for persistence purposes. Moreover, the agent can read/write the file system, e.g., navigating through folders, creating new files, and deleting existing ones. It can also create new user-level processes to execute commands, such as simulating fileless malware by running system binaries (e.g., PowerShell, WMI) and creating new OS resources. For example, the execution of user-mode commands can be accomplished using worker factories \cite{WorkerFactoriesBlog, WorkerFactoriesPoC}, a Windows mechanism that allows the kernel to create user-space thread pools and let them execute specific tasks.

%\vittorio{Spiegare che meccanismi vengono usati per eseguire comandi user mode (e kernel mode)}

%Lo emulation agent ascolta le comunicazioni dal server. Esso chiama le API del kernel come se fosse un modulo del kernel. Può accedere alle varie risorse del sistema operativo, quali ad esempio i descrittori dei processi e il registro di sistema. Queste risorse permettono anche di accedere alla intera memoria dei processi in user-level (ad esempio, il descrittore di un processo indica le regioni di memoria in cui si trovano codice e dati dei vari processi). Può sia leggere la memoria dei processi (es. process dumping, per furto di password, token e altri dati) sia modificare la memoria dei processi (es. process/DLL injection, per nascondere porzioni di codice malevolo in un processo del sistema). Può modificare il registro ai fini di persistenza. Può leggere e scrivere il filesystem, per navigare attraverso le cartelle, copiare dei file, sovrascrivere dei file esistenti, caricare dei nuovi file. Può lanciare nuovi processi in user-level per eseguire dei comandi. Ad esempio, per simulare fileless malware eseguendo programmi di sistema (es. Powershell, WMI). 



\subsection{Emulation manager}
\label{sec:emulation_manager}

The \textit{emulation manager} communicates with the agents. Its role is critical to orchestrating the low-level actions performed by the agents into emulating the complex behavior of APTs, as in the example of Section \ref{sec:background}. 
It also offers a user interface to manage Laccolith. In particular, it offers interfaces to inject agents into specific targets, to access C2 functions (e.g., listing connections to agents, sending a command to an agent, reading its output, starting an autonomous operation), to customize parameters (e.g., choosing which payload to inject), and upload and download files (e.g., to exfiltrate data and information gathering). The emulation manager is also responsible for the management of the \textit{facts}. A fact is a piece of information about the target system, helpful to run an ability. The manager communicates the fact values to emulation agents when they need specific information to perform an action. For example, suppose the goal of the emulation is to perform lateral movement to another machine in the local network. The emulation agent will perform a network scanning action, whose outcome will be a fact containing the username and IP address of the target machine. The agent will then use this fact to perform lateral movement.

%\textcolor{red}{puoi dire anche qualche parola sui "fact", e la raccolta di fact per supportare azioni successive (con un qualche esempio concreto, ad esempio l'analisi di username per fare poi lateral movement)}
%\textcolor{red}{Spiegare che emulation manager mette insieme quello che agent fa a basso livello: permette di orchestrare tutto il resto e realizzare la simulazione dell'APT}
%Lo emulation manager fornisce un interfaccia per l'utente, e comunica/coordina gli agent. Fornisce vari comandi. Vedi anche la lista di azioni indicate nella parte "framework" di Marco.

\subsection{Implementation}
\label{sec:implementation}

We implemented the design of Laccolith for the QEMU hypervisor for x86\_64 \cite{QEMU}, running on a Linux host managed by Libvirt \cite{LibVirt}, and with hardware-supported virtualization based on KVM \cite{KVM}. Laccolith runs as a privileged process on the Linux host and accesses VM memory through a virtual device file. Our implementation targets the Microsoft Windows OS as the guest OS for the victim machine. 
We selected Windows as the target OS since it is a common target for APTs and is widely used in the adversary emulation landscape. For example, the MITRE ATT\&CK framework started as a project to gather information about TTPs against Windows-based systems \cite{strom2018mitre}. 
We used Volatility \cite{Volatility}, a virtual machine introspection (VMI) framework, to get Windows kernel symbols. We chose Volatility since it is a widespread and well-known framework that offers several profiles to inspect the memory of several OSes. Using a popular VMI framework facilitates the portability of Laccolith to new versions of the guest OS (e.g., builds of Microsoft Windows) and new guest OSes since the community continuously provides multiple profiles to align VMI with new releases of the OSes. 


%Through Volatility, we were able to get the virtual addresses of the system call to inject the shellcode. The virtual address was not sufficient to perform the injection, since our injector can only write the RAM's live image using the offsets of physical addresses. To fill this \textit{semantic gap}, we retrieved the corresponding physical address for a given virtual address, based on the assumption that, if we consider a sufficient number of bits of the system call address, it is likely to be a unique sequence \cite{17}. 


%\textcolor{red}{Spiegare qui che è stato usato Linux/KVM, il discorso del file virtuale /dev/mem, Volatility, e che supportiamo Microsoft Windows come target. Spiegare che Linux/KVM e Windows sono ampiamente utilizzati nei rispettivi ruoli e sono delle buone scelte. Spiegare che Volatility è un progetto molto ampio e che fornisce profili per numerosissime versioni di Windows ed altri SO. Grazie a Volatility è molto facile applicare Laccolith su una nuova versione del guest OS o su un nuovo tipo di guest OS, perché la comunità già fornisce questi profili per vari scopi. È anche facile programmare un profile per un guest OS laddove non sia già supportato.}


\begin{comment}

\subsection{Detailed design}
\label{sec:architecture}

In this section, we introduce the architecture of the proposed approach, shown in Figure \ref{fig:Laccolith architecture}. The idea for the novel approach came from a Proof-of-Concept exploit by Google Project Zero \cite{ProjectZero}. We considered a scenario in which the attacker could compromise a hypervisor with a zero-day exploit and wanted to leverage the newly gained arbitrary read/write access to any virtual machine's RAM to inject an agent into the VM itself. The agent would then have high privilege and use it to evade defense. The existence of this type of exploit justifies the usage of virtualization technologies for adversary emulation, by performing an injection over channels that are not usually monitored by AV/EDR solutions.
The component responsible for injection, namely \textit{injector}, must have read/write access to the VM RAM in real-time and should be decoupled from the specific virtualization technology. Therefore, the idea is that this component should access the RAM not by using hypervisor-specific APIs, but by common APIs. 
Many hypervisors offer the possibility of mapping the RAM of a VM to a file. Therefore, the needed setup is to configure the hypervisor itself in such a way that the VM RAM is exposed as a file. At this point, the injector has 'physical access' to the RAM of a VM: an offset in the file corresponds to a physical address.

Since there could be performance issues with this design choice, it is possible to leverage the virtual file system’s functions to reclaim performance. In particular, in Linux, the \textit{/dev/shm} subfolder implements the concept of shared memory \cite{Cyberciti}: having the RAM file reside there is equivalent to having that file internally mapped to the hypervisor’s RAM.
%\marco{Si può anche omettere l'uso di gnome-boxes, il cui riferimento comunque è questo https://wiki.gnome.org/Apps/Boxes , perché i file XML sono nel formato definito da Libvirt; applicazioni come gnome-boxes e virtual machine manager automatizzano la creazione del file XML descritto e chiamano i binaries di Libvirt (come virsh) per validare modifiche manuali alla configurazione XML fatte dalla GUI, far partire macchine virtuali e stopparle, e così via. Come side note, Libvirt è indipendente da qemu: descrive VM in formato XML specificando anche che hypervisor utilizzare, anche se alcune configurazioni presenti nel file XML potrebbero essere hypervisor-specific. Supporta anche i container, systemd e così via. Documentazione formato di libvirt: https://libvirt.org/formatdomain.html}
To summarize, the VM RAM is mapped to a file on the hypervisor file system instead of being mapped directly to the hypervisor RAM (which is physical RAM, except in the case of nested virtualization), and that file is placed in the virtual file system which is mapped to the hypervisor RAM. So, finally, the VM RAM is still backed by the hypervisor RAM, but it is easily accessible as a file.
We used the following configuration in the architecture: the hypervisor was \textit{qemu-system-x86\_64} \cite{10}, running on a Linux host, managed by Libvirt \cite{LibVirt} and leveraging the KVM support offered by the CPU \cite{KVM}. %We used gnome-boxes \cite{gnomeboxes} as front-end: it generates an XML file to describe the domain, manage its settings, and have 'pointers' to its files (for example the hard-disk qcow2 image).
To map the RAM of the VM to a file, Qemu uses the \textit{ramfs} protocol \cite{13}. To enable it, it is compulsory to modify the generated XML file (for example with the command \textit{virsh edit $<$domain$>$}), acting on the \textit{memory backing} part.



\subsection{Injection Chain}
\label{sec:chain}
The injection chain is the set of necessary steps that, starting from arbitrary read/write access to the RAM of a VM, allows the execution of an agent with the requirements mentioned in Section \ref{sec:requirements}.

\begin{figure}[htbp]
\centering
\centerline{\includegraphics[width=\linewidth]{img/InjectionChain.png}}
\caption{Injection chain.}
\label{fig:Injection Chain}
\end{figure}




\subsubsection{The semantic gap}
\label{sec:gap}
After obtaining arbitrary read/write (R/W) access, the next step is to execute arbitrary code in a highly privileged context.

The most popular way to perform arbitrary code execution using arbitrary R/W access is by corrupting some data structures in memory to redirect the execution flow, leveraging the fact that the code will use such data structures.

Anyway, this approach is limited by the \textit{semantic gap} problem: when dealing with raw memory, the injector sees physical addresses, whereas the code sees virtual addresses. In addition to that, the code does not bypass the memory management unit (MMU), so it must always reference valid virtual addresses. So, the injector can overwrite any data structures it wants, but it does not have allocated space to place its code.
To do its job, the injector needs both physical and virtual addresses. In fact, it cannot write to a virtual address because it must write to the RAM live image at a certain offset, which is a physical address. In addition to that, it must ensure that the read and write operations it performs are not cacheable.
%\marco{Una possibile citazione per shmem2: https://github.com/rick-heig/devmem2/blob/master/shmem2.c ; ho letteralmente preso questo codice e l'ho modificato per fargli prendere un file con path assoluto ed esporre la funzionalità come uno shared object (.so) piuttosto che chiamarlo come un processo separato (per motivi di performance)}
To address this problem, we used a utility called \textit{shmem2} \cite{16} (inspired by \textit{devmem2} used in Linux to implement user-space drivers). This utility was then modified and compiled as a shared object, to be used as an external API in Python to implement custom read/write logic.
In particular, to reduce the semantic gap on system calls, we implemented a function to look up a physical address associated with a given virtual address, knowing the expected bytes at that address. The idea is that, if a sufficient number of bits of the system call code/\textbf{address} is considered, then it is likely to be a unique sequence. It is still compulsory to know the virtual address, as the least significant 12 bits of the virtual address are equal to the least significant bits of the physical address and are known as page offset \cite{17}. %\vittorio{Rifrasare chiarendo il concetto: necessario conoscere il page offset in modo tale da procedere non un byte alla volta ma 4 KB}
%\marco{Citazione per i 12 bit dell'indirizzo fisico: https://connormcgarr.github.io/paging/}
The other shade of the semantic gap is that, as mentioned previously, the injector cannot allocate space to use for the injection or rather cannot write to unallocated memory and pretend that a thread obtains a valid reference to that memory. This happens because the injector bypasses all the paging mechanisms, as mentioned earlier in this section, whereas the system does not. As an alternative, the injector could perform complex manipulations on page tables in memory and, if needed, process control blocks, to obtain the effect of making the virtual addresses already used by some processes resolve to injector-controlled physical addresses. This is a different type of attack called \textit{page table remapping attack}, and can even be used to bypass security mechanisms of \textit{enclaved execution} \cite{van2017telling}.
%\marco{Citazione relativa a page table remapping attacks ed enclaved execution: Van Bulck, Jo, et al. "Telling your secrets without page faults: Stealthy page table-based attacks on enclaved execution." Proceedings of the 26th USENIX Security Symposium. USENIX Association, 2017.}
However, this approach is over-complicated for the purpose of code execution, especially since the injector bypasses paging mechanisms. In fact, the semantic gap also gives the injector an advantage: it can use a different memory corruption strategy.
Usually, text areas of processes (where the assembly code is) are not-writeable pages. But, since the memory access is performed from the hypervisor, any byte of memory is readable and writable. As a consequence, it is possible to directly overwrite some code that will eventually be called and use it to inject an agent.
The overwritten code will be referred to as \textit{injection point} from now on.
Now there are two open questions:
\begin{itemize}
    \item Which \textbf{code to overwrite} (with high privileges) and (sub-question) \textbf{how} to find it automatically \textbf{to automate the injection}?
    \item \textbf{What to inject} there and (sub-question) how to handle the fact that it can be called multiple times?
\end{itemize}

The next sections will answer these questions, and the last section is about the engineering of the overall injection chain.


\subsubsection{Finding an injection point ("where")}
\label{sec:where}
%\vittorio{To refine}

In this section, we answer the first question posed in Section \ref{sec:gap}. In particular, since the problem of automatically finding the address of a system call has already been addressed with the combination of Volatility and the shmem2 shared object, a first target as injection point could be a generic system call. %\vittorio{chiedere conferma dell'address}

Before diving into that, it was useful to understand the process involved when a system call is issued from user mode \cite{19}. Furthermore, since the injection point needs to be easily found/adapted for different Windows versions, it is also useful to have a view of Windows x86-64 system calls by version \cite{20}.
%\marco{Citazione 19 per system calls: https://alice.climent-pommeret.red/posts/a-syscall-journey-in-the-windows-kernel/ ; Citazione 20: https://j00ru.vexillium.org/syscalls/nt/64/ ; In realtà in pratica sto riportando quelle che avevo sulla tesi, quindi per gli altri punti interrogativi continuerei a riportare queste citazioni. Ad esempio per hardware priority e funzioni disponibili per i driver faccio riferimento alla documentazione di WDK fornita da Microsoft. Il valore di IRQL pari a 0 rappresenta il PASSIVE\_LEVEL (esiste anche -1 che è IDLE).}

System calls are a good fit as injection points because they are eventually invoked by system processes. In addition to that, it is important that the chosen injection point is invoked with the right hardware priority \cite{21}. This happens because, once the agent is executing in kernel mode, it is necessary to use Windows’ internal kernel functions to perform useful actions, in particular functions available to drivers \cite{22}. From the documentation, it is possible to see that most of the functions require to be called in \textit{PASSIVE\_LEVEL}. In addition to that, we performed some reverse engineering in kernel debug to discover that the code of these functions performs the necessary checks to ensure that they are called with the right Interrupt Request Level (IRQL).

The hardware priority is inherited from 'who' invoked the specific code. When an operating system starts, it executes at the highest priority and with the highest privileges. To change its priority and lower its privileges, it must modify the status registers of the processor. These registers can be changed only with a high privilege level, meaning that an execution thread is able to drop its privileges, but cannot reclaim them. For this reason, there are special instructions that enable the call of high-privileged functions. The operating system needs to set up the handlers of these special instructions before dropping its privileges. In the case of Windows, on an abstract level, the module with the highest privileges and the highest priority is the dispatcher, responsible for the execution of all threads (both kernel and user). That is why its hardware priority level is called DISPATCH\_LEVEL. There may also be other execution threads executed at DISPATCH\_LEVEL, such as the handlers of hardware interrupts. Since this is the highest priority level, it cannot be interrupted, even by the dispatcher itself (because it runs at the same priority). Therefore, the handler of a hardware interrupt, like the routine associated with a timer, must perform its tasks quickly so it cannot, for example, issue blocking calls. By disassembling any Windows kernel function available to drivers, that cannot be called at DISPATCH\_LEVEL, it is easy to see that the first instructions perform a check about the IRQL at which the function is called, and raise a kernel exception if the IRQL is higher than expected. There are many intermediate IRQLs in the kernel, there are the hardware priorities for user mode threads and there are the hardware priorities for real-time user mode threads.  So, it is clear that the dispatcher and handlers of hardware interrupts have the highest priorities, then there is a mix of priorities of kernel threads and user threads. %\vittorio{Chiarire: gerarchia delle priorità} 
In fact, most of the kernel code has a lower priority than user code, because the system needs to be interactive and because most of the kernel code handles I/O with the file system, network, and other blocking systems. The IRQL at which this kernel code runs is the previously mentioned PASSIVE\_LEVEL. There are even lower levels than the passive one, but, to not wander, it is important to know that in PASSIVE\_LEVEL it is possible to perform blocking calls and, so, all of the Windows kernel API is available.

Back to system calls, it is easy to see, by putting a breakpoint on a system call while doing kernel debug, that they are called at PASSIVE\_LEVEL. In fact, after hitting the breakpoint, it is possible to inspect the IRQL saved by the debugger and see that its value is 0 (PASSIVE\_LEVEL) \cite{23}. This confirms the hypothesis that system calls are a good fit for the injection.

\textbf{At this point, the next step is to choose a system call to overwrite. Before that, we need to define some requirements for the \textit{malicious code}:
\begin{itemize}
    \item \textit{Space requirements}: the malicious code should be 'small enough' to fit into the system call code;
    \item \textit{Behavior requirements}: it needs to handle the case of being called multiple times and needs to somehow exit gracefully without hanging forever because user-space processes expect the system to return after a system call;
\end{itemize}}
%should be 'small enough' to be (space requirements); the malicious code also needs to handle the case of being called multiple times and needs to somehow exit gracefully without hanging forever, because user-space processes expect the system to return after a system call (behavior requirements). %\vittorio{Space requirements e behavior inquadrarli solo per il malicious code: per lo spazio non deve eccedere una certa dimensione (accennare al problema del codice delle syscall)}

\textbf{It is already clear that, for space requirements and for behavior requirements, the 'malicious code' which overwrites the system call cannot be the 'agent' itself but will be responsible for the allocation of the code region for the agent and the asynchronous execution of the agent in that area.}

For this reason, the injection is a multi-stage process, and the "malicious code" will be also referred to as \textit{first-stage shellcode} from now on and the agent will be also referred to as \textit{second-stage shellcode}.
%\marco{Visto che più avanti ci si riferisce ai requisiti della linear region of code come "third", "first", "second", potrebbe essere utile convertire la definizione della linear region of code in un punto elenco, per facilitare la lettura}
To choose the actual system call to overwrite, let us define the meaning of \textit{linear region of code} in this context. A linear region of code is a memory region that respects the following requirements:
\begin{enumerate}
    \item contains instructions that can be called like a function but does not contain other functions (so it can only be called at its starting address);
    \item every function called from the linear region must belong to the same linear region (so that code that does not belong to the linear region does not return in the middle of the linear region);
    \item the whole region must be contained in a single memory page, without crossing page boundaries.
\end{enumerate}

Ideally, the overwritten code should be a linear region of code, so it should satisfy the three aforementioned requirements.

The third requirement is necessary because otherwise the injection could not be performed reliably (contiguous pages in physical memory do not correspond to contiguous addresses in virtual memory, in general).

The first requirement is also necessary because otherwise the code would be called 'in the middle' and there would be errors such as invalid opcodes or bad memory accesses.

The second requirement is a nice-to-have: the impact of a 'return in the middle' is the same as the previously mentioned 'call in the middle', and its probability is nullified if the second requirement is satisfied. Since there is also the possibility of race conditions (overwriting the linear region of code when it is already in use), it is tolerable not to satisfy the second requirement, resulting in a \textit{semi-linear region of code} (a region that respects the first and third requirements but not the second one).

The chosen injection point must be at least a semi-linear region of code, better if linear. In addition to that, the region of code overwritten must be big enough to contain the whole first-stage shellcode.

We found a good candidate in the system call \textit{NtQueryVirtualMemory}, or rather, to be more precise, the function it calls, located 64 bytes later (at least in different Windows updates of build 19044): \textit{MmQueryVirtualMemory}. It is large around 3800 bytes and it is a linear region of code.

It is better to optimize the first-stage shellcode, anyway, to use as least of these bytes as possible, to be less intrusive.

After finding a conceivable injection point, we moved to the opposite side of the problem: instead of going bottom-up thinking about the first-stage shellcode, we focused on the second-stage shellcode.

In fact, the second-stage shellcode is what needs to be injected: the actual agent, whereas the first-stage shellcode is a ring in the injection chain and provides the 'how' the agent is going to be executed.

%At this point, it is already clear what the architecture for the novel approach looks like. it is depicted in the following diagram.
%\marco{Che diagramma?}

\subsubsection{Second-stage shellcode ("what")}
\label{sec:what}
%\vittorio{To refine}

The second-stage shellcode is the agent: it must open a connection to a C2 server and implement a set of commands to perform the actions required by adversary emulation campaigns. Furthermore, it runs in kernel mode. In this way, the second stage shellcode (but also the first stage) is very similar to a rootkit.

Much research and browsing were about finding something similar to a rootkit, but not too hard to modify and extend. With modifiability in mind, the best resource proved to be a project called SassyKitdi \cite{24}; he was the first to reverse engineer the DoublePulsar SMB backdoor, used for the EternalBlue exploit \cite{25}.

SassyKitdi creates a reverse TCP socket using Windows’ Transport Driver Interface (TDI) \cite{WindowsTDI}, then it sends the Windows version number and the memory dump of the lsass.exe process over the wire while, on the other end, a minidump is created from the received data. A minidump is a file containing a useful subset of the information contained in a crash dump file \cite{Minidump}.

The interesting thing, which makes this project more appealing than kernel-level backdoors like DoublePulsar, is the fact that SassyKitdi is not just an assembly payload, it is a Rust library designed to produce position-independent shellcode.

In fact, by fine-tuning the Rust compilation process (with cross-compilation to a Windows DLL), disabling the usage of the standard library, using a certain programming style and some useful abstractions (like specifying "extern" functions with \textit{stdcall} convention to call Windows kernel's internal functions, or by using inline assembly to implement certain functions), it is possible to use a high-level language and reliably obtain a working shellcode by extracting the startup section of the compiled DLL.

The Rust library contains definitions of Windows constants, enums, structs, signatures of functions, wrappers for complex I/O operations (in particular for IRPs \cite{26}), some rootkit techniques rewritten in Rust (like a technique to find \textit{ntoskrnl} base address, and the dynamic and “stealth” resolution of functions’ addresses from the export table \cite{27}), wrappers built upon the previously mentioned wrappers and the top module which compile itself as a shellcode (doing everything in the text area, without global area).

So, to build the second-stage shellcode, it was necessary to understand the library, modify the code, extract it from the compiled DLL using the provided utilities, and test it.

Without having the multi-stage injection chain ready, the only way to test it was to use a driver to load kernel shellcodes. It was used a driver developed by FireEye, called kscldr \cite{28}. In addition to that, since a kernel shellcode could crash the system, it was setup an environment with kernel debug, using KDNET. Actually, the kernel debug environment had already been previously set to study the behavior of system calls.

%The overall architecture of the test and debug environment is shown in the following diagram.
%\marco{Questo punto elenco non viene renderizzato bene; quando dico "the shellcode did not terminate gracefully", intendo dire che l'uscita del kernel agent provocava bug check nel kernel, forse si potrebbe specificare}
It took a significant effort to go from the original Rust code to a basic agent with \textit{echo} as the only command, because:
\begin{itemize}
    \item Rust code was not friendly, so the first thing was to understand it and the tricks that made the compiled code position-independent;
    \item SassyKitdi was tested with KVA Shadowing \cite{29} disabled, and its technique to find ntoskrnl base address did not work in presence of the KVA Shadowing's page guards: the solution was to use the hypervisor privilege to leak ntoskrnl base address (using Volatility's \textit{windows.modules} plugin) and patch the shellcode bytes before loading/injecting the shellcode;
    \item TDI operations had a hard-coded timeout of 1 second, which is too low for something executing in PASSIVE\_LEVEL: the naive solution was to increase the timeout to 15 seconds;
    \item the socket's receive handler was only a stub always sending ACK, so it took a bit of reverse engineering to understand how to modify it and develop a synchronization protocol between the shellcode's main function and the receive handler (which executes at DISPATCH\_LEVEL);
    \item the shellcode did not terminate gracefully: the termination of the kernel agent triggered a bug check in the kernel.
\end{itemize}
%\marco{Quando parlo di "common" crates non mi riferisco a quelli standard di Rust scaricabili da Internet, mi riferisco a quelli "common" nel contesto della libreria Rust fornita con SassyKitdi, potrebbe essere utile specificarlo}
After solving the previous problems, we implemented the commands of the second-stage shellcode, either by extending code from the SassyKitdi toolkit crates (a crate is a Rust package) or by creating new crates (for example to manage the file system and the system registry).

It was also compulsory to implement some functions for basic parsing of received commands, still with the requirement of the position-independent compilation (so it was not possible to use strings, because they would have gone in the global area).

For the configuration of the evasion capabilities, it was also necessary to implement a command to execute some code in user mode, i.e., a \textit{ring0-to-ring3} function. This is a common problem in rootkits, not because they want to be detected but because they want to have access to higher-level functions available in user mode \cite{30}. The command was implemented using the \textit{working factories}, the internal mechanism used to implement user-mode thread pools. The implementation was inspired by a proof of concept to go from ring0 to ring3 \cite{WorkerFactoriesBlog, WorkerFactoriesPoC}.
%\marco{Alla fine il comando user mode è stato implementato, usando le worker factories, prendendo spunto da  https://zerosum0x0.blogspot.com/2020/06/heresys-gate-kernel-zwntdll-scraping.html#workout; link giusto per PoC: https://github.com/zerosum0x0-archive/archive}

%The following diagram shows the list of implemented commands in the second-stage shellcode.

At this point, the actual agent has been implemented, but it has yet to be loaded in an automated way using the hypervisor’s privilege, rather than with a driver.

So, the next step is the implementation of the first-stage shellcode, executed after the injection from the hypervisor and responsible for the reliable loading of the second-stage shellcode.


\subsubsection{First-stage shellcode ("how")}
\label{sec:how}
%\vittorio{To refine}

This section summarizes, from a high-level perspective, the technical details of the first-stage shellcode.

The first-stage shellcode will overwrite a system call for a short period of time, long enough to communicate to the hypervisor that the area for the second-stage shellcode is ready. The hypervisor will write the second-stage shellcode to that area, then the first-stage shellcode will start a system thread to execute the second-stage shellcode and will return.

Other concurrent calls to the system call will immediately return, using some synchronization pattern. After the start of the second-stage shellcode, the original system call code can be restored.

For convenience, the first-stage shellcode is developed using the Rust library as well.

%In the following diagram, there is the hierarchical structure of the resulting “kernel shellcode library”, in which the leaves are the top-level modules that get compiled, and the other nodes are the “common crates”.

%\vittorio{Inserire diagrammi? Se sì, quali?}

%\marco{Per quanto riguarda la portabilità del first-stage shellcode, alla fine allo stato attuale il parametro "version" è "any" perché si usa volatility per ottenere le informazioni di portabilità a runtime (Windows è un sistema chiuso ma gli offset dei simboli sono scaricabili liberamente da Internet perché servono a WinDbg quando si fa kernel debug dei driver)}
The first-stage shellcode needed to be much shorter than the second-stage, so instead of finding ntoskrnl’s exported functions at run-time by iterating on the module's export table (like the second-stage shellcode does), it uses hard-coded offsets to ntoskrnl base address. The portability was implemented in the automation tool using Volatility to obtain the portability information, i.e., the symbols' offsets, at runtime.

%with a "version" configuration parameter and hard-coded offsets for a set of versions, to patch shellcode bytes at run-time before injection or to raise an exception if it is selected a version for which the portability is missing.

Since the injector sees physical addresses and the second-stage shellcode is bigger than the size of a page ($\sim$10 KB against 4 KB), the first-stage shellcode needs to allocate contiguous memory for the second-stage: this is accomplished using the function \textit{MmAllocateContiguousMemory}, from the Windows Driver Kit (WDK) \cite{22}.

So, it allocates 16 KB of contiguous memory and writes a 'very random cookie' to it, whose value is known by the injector. This cookie is called \textit{egg} because the injector must search it and overwrite it with the second-stage shellcode, which is bigger, so 'the egg hatches'.

The first-stage shellcode periodically reads the memory in which the egg is located to see if it has changed. When this happens, it means that the second-stage shellcode has been written there, so the first-stage shellcode allocates memory for a thread handle and uses the \textit{PsCreateSystemThread} function specifying the address of the area in which the second-stage shellcode is located as \textit{StartRoutine} parameter.

The only other thing the first-stage shellcode must implement is the synchronization pattern to handle concurrent calls: it must ensure that its main function is executed once and only once.

To do that, it implements a fast function to \textit{try to acquire} a spinlock, using the \textit{xchg} instruction in inline assembly \cite{31}. 'Try to acquire' means that the function does not wait on the spinlock: it returns True if it managed to enter the critical section, otherwise it returns False. When it returns True, then the first-stage shellcode’s main function must be executed, otherwise, it immediately returns.

Lo spinlock serve a gestire il fatto che il main deve essere chiamato una e una sola volta, attraverso xchg non faccio attesa attiva
Lo spinlock viene sempre mantenuto in modo tale da evitare le chiamate concorrenti

But where is the spinlock located?

Usually, when multiple threads need synchronization, the thread that starts them allocates the necessary synchronization objects: in fact, if each thread allocated objects on its own, they would be different objects. To solve this problem, since there are no pre-allocated synchronization objects, it is necessary to use an allocation primitive which is able to return pointers to the same memory area. So, physical addresses must be specified as input parameters of this allocation primitive. In Windows, the function satisfying these requirements is \textit{MmMapIoSpace}.

Which physical address to use?

A good candidate is the physical address 0x0 because it is used for early boot operations and left 'uninitialized' after that. In fact, the platform firmware usually allows operating systems to use the first KB of physical memory as a physical memory pool available to the OS for internal operations \cite{32}.

So, the solution is to map the spinlock to physical address 0x0, and the xchg operation is done by using a cookie (0xDEAD) that is unlikely to be the value at physical address 0x0 when the first-stage shellcode is called for the first time. We used a cookie because the value is uninitialized, so the code for synchronization must not check that the value exchanged was equal to a certain value, it must check that the value was different from 0xDEAD: if it is different, then the code is allowed to enter the critical section.

The first test of the injection chain was done by using the sequence \textit{int3; ret} as the second-stage shellcode, and the chain worked (the breakpoint was hit).

Since the second-stage shellcode is started with \textit{PsCreateSystemThread}, it must terminate with \textit{PsTerminateSystemThread}: this is an integration step between the first-stage shellcode and the second-stage shellcode.

This approach does not have a 100\% probability of success. Factors of unreliability and the related empirical study to estimate the success rate are reported in Section \ref{sec:experiment}.


\subsubsection{Automation}
\label{sec:automation}
\vittorio{To do}

\subsection{Versions used in development \& tests}
\label{sec:versions}
\vittorio{Eliminare?}

\end{comment}


==> tex/old/table.tex <==

%\begin{table*}[!ht]
%\centering
%\caption{\revision{Network fault models used in the state-of-the-art}}
%\label{tab:related_summary}
%\resizebox{2\columnwidth}{!}{%
%\sffamily 
%\footnotesize 
%\begin{tabular}{|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|}
%\hline 
%\rowcolor{blue!8}

\begin{table*}[ht!]
\caption{Adversary emulation solutions comparison.}
\label{tab:Tools comparison}
\resizebox{\textwidth}{!}{%
%\sffamily 
\footnotesize 
%\setstretch{0.90}
%\begin{tabular}{>{\centering}m{2.5cm}>{\centering}m{3.5cm}>{\centering}m{2cm}>{\centering}m{3cm}>{\centering}m{1.4cm}>{\centering}m{3cm}>{\centering}m{5cm}}
{\color{black}\begin{tabular}[h!]{ccccccc}
\toprule
\normalsize\textbf{Tool}  & 
\normalsize\textbf{C2 Server} &
\normalsize\textbf{Complex Attacks} &
% Built-in
% Custom
% None
\normalsize\textbf{ATT\&CK Tactics Coverage} &
\normalsize\textbf{Needs Pre-Installed Agent} &
% True
% False

\normalsize\textbf{Anti-detection} \\ \toprule

CALDERA & 
    \normalsize\ding{51} 
    & 
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.06\columnwidth]{img/table/Custom.png} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Lateral Movement.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png}
    %&
     
    &
    \normalsize\ding{51}
    &
    \normalsize\ding{55}
    \\ \midrule

Atomic Red Team & 
    \normalsize\ding{55} 
    &  
    \normalsize\ding{55} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Impact.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Initial Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Lateral Movement.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png} 
    %&
    %\normalsize277 
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule

Red Team Automation & 
    \normalsize\ding{55} 
    & 
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.06\columnwidth]{img/table/Custom.png} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Lateral Movement.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png}
    %&
     
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule

APTSimulator & 
    \normalsize\ding{55} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.06\columnwidth]{img/table/Custom.png} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png}  
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    %&
     
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule

Infection Monkey & 
    
    \normalsize\ding{51} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Lateral Movement.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png}
    %&
     
    &
    \normalsize\ding{51}
    &
    \normalsize\ding{55}
    \\ \midrule

Metta & 
    \normalsize\ding{55} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    %&
    
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule


DumpsterFire & 
    \normalsize\ding{55} &

    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.06\columnwidth]{img/table/Custom.png} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png} 
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule
    
Invoke-Adversary & 
    \normalsize\ding{55} 
    &
    \normalsize\ding{55}
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    %&
     
    &
    \normalsize\ding{55}
    &
    \normalsize\ding{55}
    \\ \midrule

Sliver & 
    \normalsize\ding{51} 
    &
    \normalsize\ding{55}
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Void.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png}  
    %&
     
    &
    \normalsize\ding{51}
    &
    \normalsize\ding{55}
    \\ \midrule\midrule
    
\textbf{Laccolith} & 
    \normalsize\ding{51} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/Built in.png}
    \includegraphics[width=0.06\columnwidth]{img/table/Custom.png} 
    &
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Collection.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Credential Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Defense Evasion.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Discovery.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Execution.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Exfiltration.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Impact.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Initial Access.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Lateral Movement.png}
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Persistence.png} 
    \includegraphics[width=0.065\columnwidth]{img/table/tactics/Privilege Escalation.png} 
    %&

    &
    \normalsize\ding{55}
    &
    \normalsize\ding{51}
    \\ \bottomrule
    
\end{tabular}}
}%

\includegraphics[width=1.25\columnwidth]{img/Legenda.png}

\end{table*}

